A Survey on Automated Log Analysis for Reliability Engineering

Logs are semi-structured text generated by logging statements in software source code. In recent decades, software logs have become imperative in the reliability assurance mechanism of many software systems because they are often the only data available that record software runtime information. As modern software is evolving into a large scale, the volume of logs has increased rapidly. To enable effective and efficient usage of modern software logs in reliability engineering, a number of studies have been conducted on automated log analysis. This survey presents a detailed overview of automated log analysis research, including how to automate and assist the writing of logging statements, how to compress logs, how to parse logs into structured event templates, and how to employ logs to detect anomalies, predict failures, and facilitate diagnosis. Additionally, we survey work that releases open-source toolkits and datasets. Based on the discussion of the recent advances, we present several promising future directions toward real-world and next-generation automated log analysis.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> [CSUR 2020] Log Survey/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> [CSUR 2020] Log Survey/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> [CSUR 2020] Log Survey/sections/best_practices.tex <==
\section{Best Current Practices}
\label{sec:best_practice}
Log plays an essential role in industrial companies for its carried information, e.g., log management tools have been integrated in various cloud platforms. Although this survey is mainly research-oriented, in this section, we intend to discuss the current industrial best practices based on our experience and surveyed papers and articles. Note that the practices do not indicate the underlying technologies used by specific companies and we do not aim to include all the best practices.
Most existing practices concentrate on the logging, log collection, and monitoring aspects, which are summarized into six best practices as follows. 

% only research at a glance (e.g. search the web with keywords like "log practice", "logging practice") and 

% Due to the high confidentiality of industrial logs, detailed descriptions about logging practices are often unavailable. Therefore, we could collect the common practices from public blogs, documents and publications. 

% \subsection{Logging}
\paragraph{Practice 1: Always follow the logging standards} It is crucial to follow the standards of logging during development, otherwise the produced logs would be hard to maintain, search and analyze. For example, the following logging standards are shared by various systems: (1) Timestamp: timestamp helps developers understand the sequential relationship among log events. Using correct timestamps (UTC/timezone adjusted) is necessary for debugging and analytic purposes. (2) Verbosity levels: proper verbosity levels ease log parsing and searching. In addition, aggregating logs by verbosity level is beneficial. (3) Format: log format is highly correlated with the parse and search procedures while most people might ignore. It is recommended to structure logs following an agreed standard (e.g., in JSON format) within the same project group. (4) Log message:  meaningful log messages facilitates the identification of the correct root cause for a failure. To construct meaning log messages, it is suggested to avoid duplicate logging descriptions (e.g., by assignment a unique ID to each logging statement).

\paragraph{Practice 2: Keep proper quantity of log messages}
Controlling the number of logging statements in the source code is very tricky. If logging too little, we may not have adequate information for problem diagnosis. On the contrary, if logging too much, we can easily get overwhelmed by the huge volume of logs and problem diagnosis is like looking for needles in haystacks. Moreover, too many logging statements could lead to unnecessary performance overhead~\cite{DBLP:conf/osdi/YuanPHLLTZS12, DBLP:conf/usenix/DingZLZLFZX15}. Hence, it is crucial to keep proper quantity of log messages.

% Generally, the logging practices are in align with key components in logs: 

% \subsection{Log Collection}
\paragraph{Practice 3: Trace log cycle across services} 
The widely-employed micro-services and components in industry bring great challenges to the tracing of a request life cycle. Engineers may get overwhelmed by interleaving logs generated by different requests, hindering problem diagnosis in practice. Therefore, it is necessary to record the event ID information during log collection. A recent study~\cite{lou2017experience} revealed that many difﬁculties in automated log analysis are caused by logs of low quality, and a typical example is the missing of event IDs. Without event IDs, we cannot link log messages related to the operations of a single request together. Event ID is also widely leveraged in recent research work~\cite{xu2009detecting, he2018identifying, logcluster15}. Typically, developers add a unique event ID to the head of each log message, and use it during the inter-service communications.

\paragraph{Practice 4: Aggregate logs to a centralized location}
Since logs are often generated in different services and components separately, it is important to aggregate the logs to a centralized location for convenient log search and analysis. Moreover, there are many practical challenges to consider after aggregating logs, including log file name configuration, retention policy, storage size, backup strategy, etc. We take retention policy as an example. The increasing volume of log data boost the storage cost and query time, thereby an appropriate retention policy is highly in demand. In addition, logs of different types might have different retention requirements. For example, application logs for troubleshooting can be kept for only a few weeks, while audit logs or transaction logs require much longer retention times. Therefore, the retention policy should be flexible. 

    
\paragraph{Practice 5: Safeguard the collected logs}
Due to the abundant information (e.g., database address) stored in logs, log data is often under a high risk of attacks. Adversaries tend to remove their trails of action, and an intuitive way is to remove any logs that might reveal their actions. Therefore, safeguarding the log files in case of an attack is a must. Because of similar reasons, industrial companies are usually not willing to share their log data to the public. Apart from setting up proper safeguarding strategies for the log storage, it is a highly-desirable practice to avoid logging any confidential information (e.g., password). Recording suspicious human activities (e.g., failed authentication) and system behaviors (e.g., spikes in resource consumption) are also crucial to log safeguarding. 


\paragraph{Practice 6: Integrate logs with monitoring metrics}
In a large log dataset, manually inspecting every log message brings heavy workload to the developers. The log information is useful only when an issue is identified. In practice, logs are often used together with other signals such as monitors. A monitor  aggregates information from multiple sources and often serves as the first step towards troubleshooting. The monitoring metric could be a status count extracted from raw logs (e.g., the number of error events), a health indicator of service performance (e.g., the number of successful requests) or a resource monitor (e.g., CPU and memory consumption). Generally, monitors are embedded in a monitoring dashboard for real-time monitoring and alerting. Because of these monitors, troubleshooting by searching and analyzing logs becomes more effective.




 



==> [CSUR 2020] Log Survey/sections/failure_diagnosis.tex <==
\subsection{Failure Diagnosis}
\label{sec:log_failure_diagnosis}
\subsubsection{Problem Formulation} Unlike anomaly detection and failure prediction that are usually formalized as a classification task, failure diagnosis targets to identify the underlying causes leading to a failure that has affected end users. It is often closely related to the root cause analysis.
Specifically, although anomaly detection and failure prediction can pinpoint whether a problem occurs or will occur, there is a huge gap between the detection and removal of a problem or a failure. To completely resolve the problems, failure diagnosis is a crucial step, but the diagnosis process is notoriously expensive and inefficient. It is reported that failure diagnosis takes over $100$ billion dollars, and developers spend more than half of their time on debugging~\cite{zhang2019inflection}. Following the concept of error, fault, and failure, as defined in~\cite{laprie1995dependable}, failure diagnosis aims to identify the fault that has led to the user-perceived impairment in a software system. In the broad domain of failure diagnosis, log-based failure diagnosis is now a standard practice for software developers.
% Due to the complexity of software systems, failure diagnosis is often realized by experienced developers and requires a large amount of manual efforts. 
However, failure diagnosis is very challenging. The complexity of modern software systems grows rapidly, where different services, software, and hardware are tightly coupled. It is too complex to correctly and efficiently disentangle the relations among the fault, failure, and human-observed symptoms. 
% For example, an application failure might come from a fault in the storage system caused by a hardware problem. 
Moreover, as software systems become more mature, failures are becoming more and more hard to detect and diagnose, from perceptible software functionality issues to imperceptible problems~\cite{kavulya2012failure}, \textit{e.g.}, performance issues~\cite{aguilera2003performance, mi2013toward, yu2014comprehending}.


To tackle these challenges, in recent decades, techniques to automate the diagnosis process have been widely developed, for example, using the informative logs~\cite{chuah2010diagnosing, jiang2017causes, zhou2019latent}. Jiang \textit{et al.}~\cite{jiang2009understanding} provided one of the first characteristic studies of log-based problem troubleshooting on real-world cases. They concluded that problem troubleshooting is time-consuming and challenging, which can be significantly facilitated by logs. In addition, they appealed to engineers to employ automated methods to speedup the problem resolution time, which is also the focus of this survey. Likewise, Zhou \textit{et al.}~\cite{zhou2018fault} empirically investigated the faults and debugging practices in microservice systems. The results show that proper tracing and visualization techniques can improve the diagnosis, which also suggest the strong needs for more intelligent log analysis. Other empirical studies include understanding failures with logs in high-performance computing (HPC) systems~\cite{el2013reading}, cloud management systems~\cite{cotroneo2019bad}, web servers~\cite{huynh2009another} and industrial air traffic control system~\cite{cinque2014logs}.


In this section, we review recent work on automated log-based failure diagnosis. Particularly, these research studies mainly focus on the large-scale software systems where failure diagnosis is burdensome, such as general distributed systems, storage systems, big data systems, microservice systems. As the characteristic and functionality may vary, these systems demonstrate different failure behaviors. However, the overall methodology for failure diagnosis still shares similar techniques, which can be categorized into four types, \textit{i.e.}, execution replay, model-based, statistics-based, 
and retrieval-based methods. There are also studies on diagnosing the hardware fault by traces (\textit{e.g.}, \cite{li2008trace}), which are beyond the scope of this survey.

\subsubsection{Execution Replay Methods}
Traditional rule-based methods heavily rely on a set of predefined rules (\textit{e.g.}, in the format of "if-then") from the expert knowledge to diagnose failures. However, the methods cannot be well generalized to unseen failures that are not included in the rules. On the contrary, execution replay methods aim to automatically infer the execution flow from logs and trace back to the software system failure, as previously introduced in Section~\ref{sec:log_mining_workflow}. The set of methods is human-interpretable and automated. Yuan \textit{et al.}~\cite{yuan2010sherlog} proposed the SherLog, which analyzes source code by run-time logs to represent the detailed execution process of a failure. Specifically, SherLog infers both control and data value information of a failed execution to help developers understand the failure. Similarly, LogMap~\cite{chen2019empirical} first retrieves log messages from bug reports and then applies static analysis technique to identify corresponding logging lines in source code. At last, it traverses through logging lines to derive the potential code paths, which help reconstruct the execution path and assist the debugging process. 

\subsubsection{Model-based Methods.} Model-based methods utilize logs to build the reference model (\textit{e.g.}, execution path) for a software system and then check which log events violate the reference model. In short, it sets up standards for normal software system executions and diagnoses failures by detecting the possible inconsistency. The majority of existing model-based studies leverage the log information to reconstruct the system execution flow as a graph representation~\cite{babenko2009ava, jia2017approach, jia2017logsed}. To achieve so, Jia et al. proposed to mine a time-weighted control flow graphs (TCFG)~\cite{jia2017logsed} and the service topology~\cite{jia2017approach} from interleaved logs during the offline phase. In the online phase, a failure can be easily diagnosed by observing the deviation between execution log sequences and the mined graph models. After observing that log sequences generated by a normal execution are consistent across multiple runs, Tak \textit{et al.}~\cite{tak2016logan} proposed the LOGAN to capture normal log patterns by log grouping, log parsing, and log alignment. When a failure occurs, LOGAN highlights the divergence of current log sequence from a reference model and suggests the possible root cause. Different from these research tasks, to detect concurrency bugs in distributed systems, Lu \textit{et al.}~\cite{lu2018cloudraid} proposed to mine logs from historical executions to uncover feasible but undertested log message orders. The log message orders represent possible execution flow that are likely to expose errors.


\subsubsection{Statistics-based Methods.} Since software systems generate logs to record normal and abnormal executions, it is intuitive to employ some statistical techniques (\textit{e.g.}, statistical distribution, correlation analysis) to capture the relationships between logs and the consequent failures.

Chuah \textit{et al.}~\cite{chuah2010diagnosing} developed a diagnostics tool, FDiag, to parse the log messages and employs statistical correlation analysis to attribute the observed failure to a possible root cause. However, the diagnostic capability of the proposed method is limited to known failures. To overcome the difficulty, Chuah \textit{et al.}~\cite{chuah2015insights} further extended their approach to an advanced FDiagV3 method, in which a PCA and ICA-based correlation approach is additionally employed. Differently, FDiagV3 can identify those unknown failures by automatically extracting the outlier issues. In~\cite{fu2014digging}, a three-step approach is designed to establish the causal dependency graph through log events, which helps identify the process that a failure occurs. The general idea resembles execution replay methods, but the causal dependency graph is statistically mined by grouping similar log events and utilizing the temporal order information. Similarly, Yu \textit{et al.}~\cite{yu2014comprehending} proposed to comprehend performance problem of device drivers in Windows. The method narrows down the diagnosis scope and pattern mining by measuring the impact of suspicious components on performance and representing the behavior pattern with the signature set tuple. Then, thresholds are set to identify highly suspicious and high-impact components that are likely to cause performance problems. 


Lu \textit{et al.}~\cite{lu2017log} proposed to detect and diagnose anomalies in the Spark system. In complementary to previous studies, the proposed method builds statistical models from the data distribution of several task-related features. It then diagnoses the anomaly by setting threshold and analyzes the root causes with weighted factors. Similar to Xu et al.~\cite{xu2009detecting}, SCMiner~\cite{zaman2019scminer} was proposed to utilize a PCA method to detect abnormal system call sequences. Then, it maps the abnormal sequence to application functions by frequent pattern mining on system call traces.  At last, SCMiner identifies and ranks buggy functions by matching with the function call traces. Likewise, CloudDiag~\cite{mi2013toward} employs a statistical technique (\textit{i.e.}, based on the data distribution) to identify the category of a fine-grained performance problem. Then, a fast matrix recovery algorithm, RPCA, is adopted to identify the root cause (\textit{i.e.}, method invocations) for the performance failure. 



\subsubsection{Retrieval-based Methods.} In practice, failures that previously occurred are valuable since they can aid developers in better diagnosing newly-occurred failures. Retrieval-based methods, as indicated by the name, retrieve similar failures in a knowledge base composed of failures in history or populated by injected faults in the test environment.
Shang \textit{et al.}~\cite{shang2013assisting} focused on diagnosing big data analytics applications in Hadoop system by injecting failures manually and analyzing the logs. Particularly, they proposed to uncover differences between pseudo and cloud deployments by log parsing, execution sequence recovery, and sequence comparison. 
Pham \textit{et al.}~\cite{pham2016failure} adopted a similar idea but they targeted on the general distributed system. Under the assumption that similar faults generate similar failures, we can locate the root cause of a reported failure by inspecting matched failures in the knowledge base. The method first reconstructs execution flows between system components, computes the similarity of the reconstructed flows, and performs precise fault injection. Nagaraj \textit{et al.}~\cite{nagaraj2012structured} proposed to diagnose the performance failures by comparing the logs of system behaviors in good and bad performance. Based on the two collected sets of logs, they applied a number of machine learning techniques to automatically compare and infer the strongest associations between performance and system components, where failures were likely to happen.


Similarly, CAM~\cite{jiang2017causes} applies the same idea to the cause analysis for test alarms in system and integration testing. In detail, the failure matching is achieved by using the K nearest neighbors (KNN) algorithm to find similar attribute vectors, which are built on test log terms extracted by term frequency–inverse document frequency (TF-IDF). 
Furthermore, Amar et al~\cite{amar2019mining} extended the CAM by keeping failing logs and removing logs that passed the test. Then, the most relevant logs in historical failures were extracted by a modified TF-IDF and then vectorized. The vectors were utilized to train an exclusive version of KNN to identify possible log lines that led to the failure. Yuan \textit{et al.}~\cite{yuan2019approach} facilitated the failure diagnosis by leveraging historical failures. They built four classifiers by vectorizing historical failures logs using natural language processing techniques. When a new failure occurs, the corresponding classifier was employed to identify the root cause. Moreover, some failures are indistinguishable because they generate very similar logs. To tackle the problem, Ikeuchi et al. ~\cite{ikeuchi2018root} proposed to utilize user actions. At first, a log-based failure database is constructed by performing various user actions. In the online deployment phase, when a user action is performed, operators match the failures with the database to identify the root cause.


 

% \subsubsection{Classification-based methods.}
% The line of research is intuitive as it builds machine learning models to determine the root causes that distinguish the normal execution and failures. Hence, these methods are often supervised and require a large amount of labels to perform well. 

%  Similarly, MEPFL~\cite{zhou2019latent} trains textcolor{red}{machine learning models} at both the trace level and the microservice level by utilized a number of features defined on the system trace logs. Three different models are trained on logs that are collected from automatic executions of the microservice application and its faulty versions produced by fault injection. During the inference phase, the models can predict latent errors, relevant microservices, and fault types, respectively.




==> [CSUR 2020] Log Survey/sections/future.tex <==
\section{Future Directions}\label{sec:future}
In this section, we would like to discuss promising future directions.
Particularly, we start with concluding future directions for each topic reviewed in this survey: logging, log compression, log parsing, and log mining. Then we share our thoughts on the next-generation log analysis framework, which might shed light on future studies. In particular, we believe the next-generation log analysis should be ``autopilot" via better human-computer interaction and an end-to-end analytic structure. Note that these directions are mainly recommended by the authors or reviewers of this paper and we believe there are much more interesting topics beyond what we have discussed in the following.

% At last, since log analysis has a high practical value and depends heavily on the real-world datasets, we will talk about how to promote the industry-academia collaborations, help both the healthy development of the academic research and the practical deployment of the proposed techniques.

% Automated log analysis for reliability engineering has been rapidly developed in the past decades, as reviewed in this survey. In the near future, we expect more interesting and inspiring research studies in the automated log analysis field. 

\subsection*{Logging}

Although logging has been widely studied in recent years, we believe there is still much room for further improvement. In the following, we introduce two future directions: analysis-oriented logging and logging convention enforcement.

\label{sec:logging_future}
\subsubsection*{Analysis-Oriented Logging.} As the foundation of automated log analysis, current logging practices mostly focus on characterization and recommendation of logging statements (\textit{i.e.}, where, what, and how to log). Meanwhile, a recent industrial study~\cite{DBLP:conf/icse/BarikDDF16} pointed out that the inconsistent presentation format with-in and among teams poses a significant challenge in developing automated log analysis tools. In addition, even an effective log mining algorithm could generate meaningless results if the software runtime information is not well-documented in the collected logs. Thus, a crucial direction is designing advanced logging mechanisms that can coordinate with the subsequent log analysis steps during the development.

\subsubsection*{Logging Convention Enforcement} Although there are no golden rules of logging, developers typically intend to have consistent logging practice in the same project. For example, senior developers in a project may define a set of rules with examples and ask other developers to follow. However, it is difficult for junior developers to get familiar with all the suggested rules, which often change when they are involved in new projects. Thus, it is promising to design automated tools (e.g., lightweight static analysis tools) to recommend logging practice and report potential violations of the "missing"/"incorrect" logging code.


%  \subsubsection*{Analysis Oriented Logging.} Section~\ref{sec:log_mining} has demonstrated that the value of logs in automatically mining patterns and diagnosing failures. A recent industrial study~\cite{DBLP:conf/icse/BarikDDF16} pointed out that the inconsistent presentation format with-in and among teams poses significant challenges in developing automated log analysis tools. Hence, an interesting research direction is to design advanced logging mechanisms that can coordinate with the subsequent log analysis steps during the development.

% \subsubsection*{Automated Generation of Logging Statements.} The automated generation of logging statements can alleviate developers' burden. Recent research at the intersection of machine learning, programming languages, and software engineering has taken an important step toward proposing learnable code-generating models that utilize rich patterns in source code~\cite{DBLP:journals/csur/AllamanisBDS18}. Automatically generating logging statements is approachable by incorporating code-generating models with existing approaches that suggest where, what, and how to log.

% \vspace{0.2em}
% \noindent\emph{Analysis Oriented Logging.} Section~\ref{sec:log_mining} demonstrated that the value of logs in automatically mining patterns and diagnosing failures. A recent industrial study~\cite{DBLP:conf/icse/BarikDDF16} pointed out that the inconsistent presentation format with-in and among teams poses significant challenges in developing automated log analysis tools. Hence, an interesting research direction is to design advanced logging mechanisms that can coordinate with the subsequent log analysis steps during the development for better analysis.

% % \vspace{0.2em}
% \noindent\emph{Automated Generation of Logging Statements.} The automated generation of logging statements can alleviate developers' burden. Recent research at the intersection of machine learning, programming languages, and software engineering has taken an important step toward proposing learnable code-generating models that utilize rich patterns in source code~\cite{DBLP:journals/csur/AllamanisBDS18}. Automatically generating logging statements is approachable by incorporating code-generating models with existing approaches that suggest where, what, and how to log.


\subsection*{Log Compression}
% Although log compression has been studied for decades, its performance is still unsatisfactory in varying storage and practical use demands. We summarize the future directions on automated log compression and query-efficient log compression.
% \begin{itemize}
% \subsubsection*{Automated Log Compression.} Existing log compressors often require many heuristic rules and cannot be generalized well to other log data~\cite{balakrishnan2006lossless, hassan2008industrial, deorowicz2008sub}, which makes a general log compressor inefficiently designed. To tackle the problem, a fully automated log compression algorithm is highly in demand. It should be automatically adapted for different log formats and require few heuristic rules. One possible solution is to use machine learning techniques to uncover the redundant log patterns and then compress the redundancy respectively.

\subsubsection*{Query-efficient Log Compression.} Different logs may play different roles and have different storage requirements. For example, failure logs could be frequently queried by developers and the corresponding log compressor should promptly respond to the query request. Therefore, how to incorporate the query demands into log compression becomes vital to log service providers. Particularly, several potential sub-problems could be: how to predict the user query request, how to store logs in a systematically modularized way for different demands, etc.




\subsection*{Log Parsing}
% Although there have been much progress in log parsing in recent years, we find it still have a lot of room for further improvement. In this section, we present our insights and suggestions on heterogeneous log parsing and distributed online log parsing.


% \subsubsection*{Heterogeneous Log Parsing.} Most existing log parsers assume that log messages of a system should have the same headers (\textit{e.g.}, timestamp and component name), which are often extracted before hand by ad-hoc scripts. However, modern software is very complex and often adopts different logging frameworks, leading to a mixture of log messages with different headers, consequently degrading the performance of existing approaches. Therefore, a log parsing method that can automatically extract the header of log messages is called for.

\subsubsection*{Distributed Online Log Parsing.} Existing approaches~\cite{He2017TDSC, DuTKDE18} provide offline parallel mechanisms to accelerate the log parsing process. However, there is a lack of distributed online parsing solution in large-scale distributed systems. The desired log parser should have multiple running threads in both the master and the working nodes and parse the log messages in a streaming manner. A trade-off will be considered between parsing accuracy and efficiency via an event template synchronization mechanism. With a distributed online parser, we could generate structured log messages on the fly, which facilities both log compression and log mining tasks.
% Each thread should maintain its own parsing rules (\textit{e.g.}, a list of regexs) and synchronize with other threads in an accurate and efficient way.

% \item \textbf{Human-assisting log parsing} Existing log parsing papers aim at fully automated log parsing. However, due to the flexibility of software logs, it is extremely difficult, if not impossible, to consistently achieve 100\% parsing accuracy. In particular, a constant and a variable could have the same occurring frequency, which makes log parsers difficult to tell them apart. In the future, "human-assisting" log parsing will be a promising direction. "Human-assisting" parsing includes humans in the loop and allows them to manually fix the event templates, which can be reflected in the parsing results in real-time. Towards this goal, better online parsing algorithms and human-computer interaction mechanisms will be crucial.


\subsection*{Log Mining}
Although being extensively studied, log mining is still very challenging due to complex problem definition and poor data quality in different scenarios.  
In the following, we summarize insights inspired by the surveyed papers and propose some promising future directions.
Unlike some other research topics (e.g., log parsing) that are relatively mature, log mining still leaves a lot of space to explore.

\subsubsection*{Concept Drift-adapted Log Mining.} Most of the existing approaches train models with historical log data offline. However, modern software systems continuously undergo feature upgrades and system renewal; hence, the patterns of logs may drift accordingly~\cite{zhang2019robust}. Common strategies of online updating, \textit{e.g.}, periodically retraining the model, suffer from high false positive rates, and strategies like zero-positive learning~\cite{du2019lifelong} have limited generalization ability. Online learning and incremental learning that fit the log mining scenario are appealing research directions.

% \subsubsection*{Log Mining with Semantic Understanding} Logs, as a structured language~\cite{DBLP:conf/kbse/HeCHL18}, inherit abundant semantic information. Existing studies often focus on the event representation while ignoring the semantic information embedded in logs. Recently, efforts~\cite{zhang2019robust,meng2019loganomaly,mengsemantic} have been devoted towards the automatic understanding of logs, which would be effective ways to eliminate the problems brought by log concept drift. Moreover, it can also play an important role in the automated generation of logging statements.
% With the advances of deep learning models, the semantic understanding of natural languages has achieved remarkable performance.

\subsubsection*{Interpretable Log Mining.} Whether a log analysis algorithm can provide interpretable results is vital for administrator and analysts to trust and act on the automated analysis. Some traditional machine learning algorithms possess the merit of interpretability~\cite{xu2009online,shang2013assisting,lou2010mining_a,nandi2016anomaly}. However, deep learning models, though having achieved impressive performance, are criticized as black-box oracles. Therefore, the community of log analysis should continue pursuing more explainable and trustworthy algorithms, for example, by utilizing attention mechanisms~\cite{brown2018recurrent}. 

\subsubsection*{Log Completeness} Log completeness~\cite{cohen2015have} measures whether developers have seen enough logs for different log mining tasks. Log completeness is important because (1) it facilitates measuring the reliability of the log mining results and (2) it is strongly related to the heuristics that may address the scalability issues of log mining~\cite{busany2016behavioral}. However, little work has been done on log completeness, which makes it a promising and important future direction.
 
\subsection*{Next-generation Log Analysis Framework}
Log analysis, as a core component in Artificial Intelligence for IT Operations (AIOps), is crucial to the reliability engineering of software systems. Particularly, the demand for automated log analysis draws dramatic attention as the increasing needs of cloud computing. We believe that the next-generation log analysis would be the "autopilot" in cloud environment. We list as below two major directions that the next-generation log analysis framework 
may contain.

\subsubsection*{Human-computer Interactive Log Analysis.}
Current automated log analysis research facilitates the failure diagnosis process by providing insightful decisions and clues for root cause analysis. In essence, developers are still at the core of failure diagnosis. For example, the diagnosis results should be confirmed and then debugged by developers. However, there is a lack of interactions between the advanced analysis techniques and developers-in-charge. Besides, the diagnosis process and results are seldom reused in the future log analysis. Therefore, it is interesting and promising to involve developers into the loop of automated log analysis. It will be promising to build an interactive dialogue system with automated analysis tools. The automated log analysis tools first provide suggestions to the developers for decision making. Then the developers can request for additional information of failures, and the diagnosis process with human involvement can be recorded and reused to improve the automated log analysis tools.

\subsubsection*{Intelligent and End-to-end Log Analysis.}
Current automated log analysis contains several consecutive steps, but they are not working seamlessly together. In particular, they do not form an end-to-end framework, indicating the possible loss of some critical information in the middle. In our vision, the ultimate goal of the next generation log analysis is an intelligent and end-to-end framework. In this framework, logging statements are automatically suggested by considering the failure diagnosis demand and the potential machine learning models used in log mining. Then, the framework intelligently stores raw logs following practical requirements. Logs are processed without information loss and are correlated with human-observable failures for diagnosis. Moreover, the framework would automatically generate failure reports by aggregating essential information 
from all analyzed system logs. It should also auto-repair the detected failures by observing experiences from human experts.  




 
% \subsection{Industry-Academia Research Collaboration}
% Logs are often collected from large-scale software systems, which are prominent in giant industrial companies such as Microsoft and Amazon. However, developers in industry might not be available for in-depth research explorations. Academic researchers are passionate in the automated log analysis area, as indicated in the rapid increase of recent publications. Unfortunately, high-quality datasets are scarce due to the huge gap between the industry and academia. We would like to point out that the research collaboration between industry and academia should be encouraged, which we believe would benefit the development of both sides. 

% Current difficulties that hinder the log analysis collaboration are mainly twofold. The first is research problem perspective. Researchers in academia might not be aware of current challenges that the industry is facing. In practice, some research problems are not in a high priority to tackle and there could be alternative methods to alleviate the issues by some engineering efforts. One typical example is the anomaly detection, which can be solved by a number of different monitoring metrics apart from logs. Another difficulty lies in the data perspective, which has been criticized for a long time. Due to confidential reasons, industrial companies are not willing to release their datasets to the public. Several strategies might be available for addressing the issue. The first method calls for the contribution to constructing a large-scale service system which can generate sufficient logs for research use. However, the built system might not represent the industrial practice. The second strategy requires an advanced method for the anonymization of logs. By transforming the logs into other format and content, industrial companies could share their datasets to the research community. The most optimal method is to encourage the reseach collaboration by in-depth communications, for example, through internship cooperation.
    
    



% \subsection{Logging}
% \label{sec:logging_future}
% Good logging practices should have both solid a theoretical foundation and practical engineering feasibility as their impacts on both industry and academia. Current practices of logging mostly focus on characterization and recommendation of logging (\textit{i.e.} where, what, how to log), but we could take a step further to analysis-oriented and automated logging.

% \begin{itemize}
%   \item \textbf{Analysis Oriented Logging.} As we demonstrated in Section~\ref{sec:log_mining}, event logs have been a valuable source for mining system behaviors. Current logging statements make heavy use of fields, such as date, message source, key/value pairs, but a recent industrial survey~\cite{DBLP:conf/icse/BarikDDF16} pointed out that the lack of a common presentation format within the same team and within different teams poses some challenges in the development of automated log analysis tools. Therefore it will be helpful if the logging statements can be designed to coordinate with the subsequent analysis steps during the development. In another word, logging and log analysis should be considered as a whole during the design of software.
%   \item \textbf{Automated Generation of Logging Statements.} The automated generation of logging statements can alleviate developers' burden. Recent research at the intersection of machine learning, programming languages, and software engineering has taken an important step toward proposing learnable code-generating models that utilize rich patterns in source code~\cite{DBLP:journals/csur/AllamanisBDS18}. Automatically generating logging statements is possible by incorporating code-generating models with existing approaches that suggests where, what, how to log.
% \end{itemize}


% \subsection{Log Compression}
% Although log compression has been studied for decades, its performance is still unsatisfactory. Many existing log compressors are either too specific to a particular log data or too dependent on heuristic rule designing, which restricts the general applicability of log compressors in various storage demands.
% \begin{itemize}
%     \item \textbf{Automated Compression}: Due to the wide application of different logging utilities and logging practices, log format may vary dramatically, which narrows down the log compressor to specific system or application logs~\cite{balakrishnan2006lossless, hassan2008industrial, deorowicz2008sub, racz2004high}. Consequently, these log compressors requires many heuristic rules and cannot be generalize to other log data, which makes the log compressor inefficiently designed. To tackle the problem, an automated log compression algorithm is highly in demand. It should require few heuristic rules and cannot be automatically adapted for different log formats. One possible solution is to uncover the redundant log patterns in an fully automated way and then compress the redundancy respectively.
    
%     \item \textbf{Query-efficient Compression}: Logs collected from different components may have different roles in the problem troubleshooting and auditing. Some logs are stored only for record purpose while the other logs could be frequently queried by developers. For the latter, the log compression and decompression should be very efficient to instantly respond to the query request. To deal with the requirement, how to incorporate the query demands into the log compression becomes vital to log service providers. Particularly, it could be further separated into several sub-problems: how to predict the user query request, how to store the logs in a more modularized manner, how large is the log compression unit? etc.
% \end{itemize}



% \subsection{Log Parsing}

% Although there have been much progress in log parsing in recent years, we find it still have a lot of room for further improvement. In this section, we summarize our insights and the corresponding further directions in this field.

% \begin{itemize}
% \item \textbf{Log messages from different logging frameworks} Most of the existing log parsers assume that the log messages of a system should have the same header (\textit{e.g.}, timestamp and component name). Based on this assumption, the header of the log messages are often extracted before hand by ad-hoc scripts. However, modern software can be very complex, consisting of components that adopt different logging frameworks. Thus, log messages with different headers could be mixed-up in practice, intensively degrading the performance of the existing approaches. Thus, a log parsing approach that could automatically extract the headers of the log messages is in high demand.

% \item \textbf{Distributed online log parsing} Most of the existing log parsers work on a single machine. Thus, its efficiency is bounded by the device. POP~\cite{He2017TDSC} and Spell~\cite{DuTKDE18} provide offline distributed/parallel mechanism to accelerate the parsing process. However, currently, log collection and transmission incurs much overhead in large-scale distributed systems. Thus, there is a lack of distributed online parsing solution for these kind of systems. In particular, a distributed online log parser should have multiple running thread in either the master node or a working node and parse the log messages in a streaming manner. Each thread should maintain its own parsing rules (\textit{e.g.}, a list of regexs) and synchronize with other threads in an accurate and efficient way. With a distributed online parser, we could generate structured log messages on the fly, which facilities both preceding log compression step and the succeeding log mining tasks.

% \item \textbf{Human-assisting log parsing} Existing log parsing papers aim at fully automated log parsing: (1) the structured log messages should be directly used by the downstream tasks and (2) the event templates can be automatically transformed into regexs. However, due to the flexibility of software logs, it is extremely difficult, if not impossible, to consistently achieve 100\% parsing accuracy. In particular, a constant and a variable could have the same occurring frequency, which makes log parsers difficult to tell them apart. In the future, "human-assisting" log parsing will be a promising direction. "Human-assisting" parsing includes humans in the loop and allows them to manually fix the event templates, which can be reflected in the parsing results in real-time. Towards this goal, better online parsing algorithms and human-computer interaction mechanisms will be crucial.
% \end{itemize}


% \subsection{Log Mining}

% We summarize the following general challenges encountered during the mining and analysis of log data.

% \begin{itemize}

% \item \textbf{Concept Drift}. Concept drift means that the statistical properties of the target variable under prediction change over time in unforeseen manners. Such issues can also be observed in log analysis. Today's software systems continuously undergo feature upgrade and system renewal. Particularly, with the addition, removal, and modification of software's logging statements, the patterns of logs may drift accordingly, posing requirements on log mining algorithms to adapt to such pattern evolution~\cite{zhang2019robust}. However, most of the existing algorithms conduct model training with historical collected log data in an offline fashion. Common strategies of online updating include: 1) periodically retrain the model; 2) fine-tune the model when false positives are identified, which still rely largely on human intervention and suffer from high false positive rate. Moreover, they often adopt the strategy of zero-positive learning~\cite{du2019lifelong}, which trains the model without the presence of positive samples. The generalization ability of the model is therefore limited. Online learning and incremental learning that fit the log mining scenario are in high demand.

% \item \textbf{Semantic understanding}. With the advances of deep learning models, the semantic understanding of natural languages has achieved remarkable performance. Log, as a more structured language~\cite{DBLP:conf/kbse/HeCHL18}, also contain a certain level of semantics. Efforts~\cite{zhang2019robust,meng2019loganomaly,mengsemantic} have been devoted towards the automatic understanding of logs, which would be effective ways to eliminate the problems brought by log concept drift. Moreover, it can also play an important role in the automated generation of logging statements (Section~\ref{sec:logging_future}).

% \item \textbf{Interpretability}. Whether a log analysis algorithm can provide interpretable result is vital for administrator and analyst to trust and act on the automated analysis. Some traditional machine learning algorithms possess the merit of interpretability~\cite{xu2009online,shang2013assisting,lou2010mining_a,nandi2016anomaly}. However, deep learning models, though having achieved impressive performance, are criticized as black box oracles. In recent years, the proliferation of attention mechanisms~\cite{brown2018recurrent} have been demonstrated to help explain such models. However, the community of log study should continue pursuing more explainable and trustworthy algorithms that take into consideration the characteristics of modern software systems.
% \end{itemize}



% \subsection{Next-generation log analysis framework}
% Log analysis, as a core component in artificial intelligence for IT operations (AI Ops), is becoming more and more crucial to the reliability engineering of modern software systems. Particularly, the demand for log analysis draws dramatic attention as the increasing needs of cloud infrastructure and application deployment. We believe that the next-generation log analysis would be the "autopilot" in the cloud environment, which must be more automated and intelligent and involves little human intervention. We list as below several dimensions that the next-generation log analysis framework should perform well.


% \paragraph{Intelligent Log Analysis.}
% Automated log analysis consists of several distinct steps, including logging, compression, parsing, and mining. Although these steps are consecutive, they do not form an end-to-end framework, in which some critical information might be lost. Hence, the next generation log analysis framework should be end-to-end. In this framework, logging statements are automatically suggested first and utilized to record software behaviors during the runtime phase. After that, following the practical demands for diagnosis, the framework stores log datasets in an intelligent manner. At last, logs are processed without information loss and correlated with human-observable failures for diagnosis. Moreover, an ideal intelligent log analysis framework should also automatically generate the failure report by aggregating essential information including logs together. Besides, it should be able to auto-repair the detected failures by observing experiences from human experts. In this intelligent log analysis, human heuristics are involved as few as possible while most decisions can be made by intelligent algorithms. 


% % \paragraph{}
% \paragraph{Human-computer Interactive Log Analysis.}
% Current automated log analysis research can help developers ease the diagnosis burden and facilitate the diagnosis process by providing insightful decisions and clues for root cause. In essence, developer is at the core of the failure diagnosis, for example, the diagnosis results have to be confirmed and then debugging is conducted by developers. However, there is a lack of interactions between the proposed techniques and the developer. Besides, the diagnosis process and results are seldom reused in the future log analysis. Therefore, it is interesting and promising to involve developers into the loop of automated log analysis. For example, by building an interactive dialogue system, automated log analysis tools first provide suggestions to developers for decision making. Then, developers can request for additional information of failures, and the diagnosis process with human involvement can be recorded and reused to improve the automated log analysis tools.

% ~\cite{chen2020survey, 
% su2017survey}

==> [CSUR 2020] Log Survey/sections/introduction.tex <==
\section{Introduction}

In the recent decades, modern software, such as search engines, instant messaging apps., and cloud systems, has been increasingly integrated into our daily lives and becomes indispensable. Most of these software systems are expected to be available on a $24\times 7$ basis. Any non-trivial downtime can lead to significant revenue loss, especially for large-scale distributed systems~\cite{downtimeAmazon,downtimeGeneral,downtimeFacebook}. For example, in 2017, a 
downtime in Amazon led to a loss of 150+ million US dollars~\cite{downtimeexample}. Thus, the reliability of modern software is of paramount importance~\cite{lyu1996handbook}.

Software logs have been widely employed in a variety of reliability assurance tasks, because they are often the only data available that record software runtime information. Additionally, logs also play an indispensable role in data-driven decision making in industry~\cite{DBLP:conf/icse/PecchiaCCC15}. In general, logs are semi-structured text printed by logging statements (\textit{e.g.}, \fixedwidth{printf()}, \fixedwidth{logger.info()}) in the source code. For example, in Fig.~\ref{fig:slf4j-example}, the two log messages are printed by the two logging statements in the source code. The first few words (\textit{e.g.}, "Wombat") of the log messages are decided by the corresponding logging framework (\textit{e.g.}, SLF4J) and they are in structured form. On the contrary, the remaining words (\textit{e.g.}, "50 degrees") are unstructured because they are written by developers to describe specific system runtime events. 

\begin{figure}
\begin{minipage}[htb]{0.83\textwidth}
\begin{lstlisting}[language=Java]
public void setTemperature(Integer temperature) {
  // ...
  logger.debug("Temperature set to {}. Old temperature was {}.", t, oldT);
  if (temperature.intValue() > 50) {
    logger.info("Temperature has risen above 50 degrees.");
  }
}
\end{lstlisting}
\end{minipage}
\\
$\Downarrow$
\\
\begin{minipage}[htb]{0.85\textwidth}
\begin{lstlisting}[]
0 [setTemperature] DEBUG Wombat - Temperature set to 61. Old temperature was 42.
0 [setTemperature] INFO Wombat - Temperature has risen above 50 degrees.
\end{lstlisting}
\end{minipage}
\caption{An example of logging statements by SLF4J and the generated logs.}
\label{fig:slf4j-example}
\vspace{-2pt}
\end{figure}

A typical log analysis management framework is illustrated by the upper part of Fig.~\ref{fig:framework}. Particularly, traditional logging practice (\textit{e.g.}, which variables to print) mainly relies on developers' domain knowledge. During system runtime, software logs are collected and compressed as normal files using file compression toolkits~\cite{liu2019logzip} (\textit{e.g.}, WinRAR). Additionally, developers leverage the collected logs in various reliability assurance tasks (\textit{i.e.}, log mining), such as anomaly detection. Decades ago, these processes were based on specific rules specified by the developers. For example, to extract specific information related to a task (\textit{e.g.}, thread ID), developers need to design regex (\textit{i.e.}, regular expression) rules for automated log parsing~\cite{he2016experience}. The traditional anomaly detection process also relies on manually constructed rules~\cite{hansen1993automated}. These log analysis techniques were effective at the beginning because most of the widely-used software systems were small and simple.





However, as modern software has become much larger in scale and more complex in structure, traditional log analysis that is mainly based on ad-hoc domain knowledge or manually constructed and maintained rules becomes inefficient and ineffective~\cite{DBLP:journals/cacm/OlinerGX12}. This brings four major challenges to modern log analysis. (1) In many practices, while a number of senior developers in the same group share some best logging practices, most of the new developers or developers from different projects write logging statements based on domain knowledge and ad-hoc designs. As a result, the quality of the runtime logs varies to a large extent. (2) The volume of software logs has increased rapidly (\textit{e.g.}, 50 GB/h~\cite{mi2013toward}). Consequently, it is much more difficult to manually dig out the rules (\textit{e.g.}, log event templates or anomalous patterns). (3) With the prevalence of Web service and source code sharing platforms (\textit{e.g.}, Github), software could be written by hundreds of global developers. Developers who should maintain the rules often have no idea of the original logging purpose, which further increases the difficulty in manual maintenance of their rules. (4) Due to the wide adoption of the agile software development concept, a new software version often comes in a short-term manner. Thus, corresponding logging statements update frequently as well (\textit{e.g.}, hundreds of new logging statements per month~\cite{weixutheis}). However, it is hard for developers to manually update the rules.


\begin{figure}[thb]
\centerline{\includegraphics[width=0.83\columnwidth]{figs/framework.pdf}}
\caption{An overall framework for automated log analysis.}
\label{fig:framework}
\vspace{-6pt}
\end{figure}

To address these challenges, a great amount of work has been accomplished by both researchers and practitioners in recent decades. In particular, starting from 2003, a line of research efforts have been contributed to automated rule construction and critical information extraction from software logs, including the first pieces of work of log parsing~\cite{vaarandi2003data}, anomaly detection~\cite{vaarandi2003data}, and failure prediction~\cite{sahoo2003critical}. In addition, in the same year, H{\"a}t{\"o}nen \textit{et al.}~\cite{hatonen2003comprehensive} proposed the first log specific compression technique. Later, many empirical studies were conducted as the first steps towards some difficult problems in automated log analysis, including the first study on failure diagnosis by Jiang \textit{et al.}~\cite{jiang2009understanding} in 2009, the first exploration of logging practice by Yuan \textit{et al.}~\cite{DBLP:conf/icse/YuanPZ12} in 2012, and the first industrial study on logging practice by Fu \textit{et al.}~\cite{DBLP:conf/icse/FuZHLDLZX14} in 2014. Recently, machine learning  and deep learning algorithms have been widely adopted by the state-of-the-art (SOTA) papers, such as the deep learning-based "what-to-log" approach~\cite{li2020wherelog} in logging practice and Deeplog~\cite{du2017deeplog} in anomaly detection. Besides machine learning, parallelization has  been employed in various recent papers, such as Logzip~\cite{liu2019logzip} in log compression and POP~\cite{He2017TDSC} in log parsing.


These extensive studies on automated log analysis across multiple core directions have largely boosted the effectiveness and efficiency of systematic usage of software logs. However, the diversity and richness of both the research directions and recent papers could inevitably hinder the non-experts who intend to understand the SOTA and propose further improvements. To address this problem, this paper surveys 158 papers in the last 23 years across a variety of topics in log analysis. The papers under exploration are mainly from top venues in three related fields: software engineering (\textit{e.g.}, ICSE), system (\textit{e.g.}, SOSP), and networking (\textit{e.g.}, NSDI). Thus, the readers can obtain a deep understanding of the advantages and limitations of the SOTA approaches, as well as taking a glance at the existing open-source toolkits and datasets. In addition, the insights and challenges summarized in the paper can help practitioners understand the 
potential usage of the automated log analysis techniques in practice and realize the gap between academy and industry in this field. We present crucial research efforts on automated log analysis from the following seven perspectives as illustrated in Fig.~\ref{fig:framework}:
\begin{itemize}
    \item Logging: Section~\ref{sec:log_practice} introduces approaches that automate or improve logging practices, including \textit{where-to-log}, \textit{what-to-log}, and \textit{how-to-log}.
    \item Log compression: Section~\ref{sec:log_compression} presents approaches to compress software logs in runtime.
    \item Log parsing: Section~\ref{sec:log_parsing} discusses how to automatically extract event templates and key parameters from software logs. 
    \item Log mining: Section~\ref{sec:log_mining} introduces what automated log mining techniques can do to enhance system reliability. We focus on three main tasks: \textit{anomaly detection}, \textit{failure prediction}, and \textit{failure diagnosis}.
    \item Open-source toolkits and datasets: Papers providing open-source toolkits and datasets, which facilitate log analysis research, are presented in Section~\ref{sec:log_tools}. 
    \item Best current practices: Supplementary A presents some common log practices in industry, which might benefit the log analysis research and industrial deployment.
    \item Future directions: Supplementary B discusses open challenges and promising future directions that can push this field forward beyond current practices.
\end{itemize}



==> [CSUR 2020] Log Survey/sections/log_compression.tex <==
\section{Log Compression}
\label{sec:log_compression}
After collecting logs by executing logging statements during runtime, logs are stored for failure diagnosis or sensitive operations auditing. Then, how to store logs efficiently becomes a challenging problem. 
Since large-scale software systems run on a 24 $\times$ 7 basis, the generated log size has been huge (\textit{e.g.}, 50 gigabytes per hour~\cite{mi2013toward}). Besides, many logs require the long-term storage for identifying duplicate problems and mining failure patterns from historical logs~\cite{yuan2019approach, amar2019mining,ding2014mining}. Auditing logs that record sensitive user operations are often stored for two years and even more to track system misuse in future. Archiving logs in such a huge volume for a long period brings inconceivably heavy burden to storage space, electrical power, and network bandwidth for transmission. To tackle these problems, a line of research has been focusing on log compression, which aims to remove the redundancy in a large log file and reduce its storage consumption. 
% In this section, we first identify challenges of log compression (Section~\ref{sec:log_compress_chall}), then shows some desired properties of log compressors (Section~\ref{sec:log_compress_prop}) and finally present research studies along the direction (Section~\ref{sec:log_compress_methods}).


\subsection{Challenges for Log Compression}\label{sec:log_compress_chall}
Practically, log compression can be achieved by various approaches. The most straightforward way is to reduce the amount of logging statements in the source code or to set a less verbose log level (e.g., change from "INFO" to "ERROR")~\cite{li2017log} in runtime. Although effective, this method leads to information loss in logs, which impedes the log-based troubleshooting. Besides, it is a common practice in existing logging libraries (\textit{e.g.}, log4j) to compress log files by some general file compressors, such as gzip. However, the method is not tailored for the semi-structured log format, making it very ineffective in log compression. The structured fields (\textit{i.e.}, constant parts) are often repetitive across many raw logs, which consume a lot of storage space and should be handled specifically. To address these issues, a tailored log compression algorithm is highly in demand. 


\subsection{Characteristics for Log Compression}
\label{sec:log_compress_prop}
An ideal log compressor should achieve a high compression ratio while imposing short compression and decompression time. The compression ratio denotes the ratio between the file sizes before and after the compression. A higher compression ratio indicates that less storage space is consumed and the compression algorithm is more effective. Additionally, log compression algorithm takes a certain amount of time to compress and decompress the file respectively, which is supposed to be as short as possible.
In this paper, we mainly explored 12 existing log compressing approaches and several empirical studies. As shown in Table~\ref{table:log_compression}, to clearly demonstrate the advantages and disadvantages of these approaches, we list several characteristics that concern the log compressors based on the following descriptions in the surveyed papers.
\textit{(1) Use of general compressors (GC).} Some log compressors utilize the general compressor as the backend technique after reformatting the logs. Specifically, these reformattings can transform raw logs to better formats that achieve a higher compression ratio. 
\textit{(2) General applicability} denotes whether the log compressor can be generally applicable to various log data formats. A general log compressor shows better utility in different scenarios. For example, as shown in the ``target data'' of Table~\ref{table:log_compression}, the log compressor proposed in~\cite{deorowicz2008sub} was specialized for Apache web log while other log compressors~\cite{christensen2013adaptive} can be applied to different log data types. 
\textit{(3) Scalability.} Since logs are often of a great volume in practice, the efficiency of log compression is crucial to the practical employment. A highly scalable compressor could save both the compression and decompression time, which thereby saves the log query time and supports real-time analysis.
\textit{(4) Heuristics.} The deployment would be more efficient and smoother if the log compressor requires little prior knowledge, \textit{e.g.}, heuristic rules on log formats and preprocessing procedures. The less heuristics a log compressor needs, the more generally applicable it would be. 

 
\begin{table}[t]
\begin{center}
\caption{Summary of log compression approaches.}
\label{table:log_compression}
 \begin{tabular}{c|c|c|c|c|c}
 \toprule
\multicolumn{2}{c|}{\bf Methods} & GC	& Target Data	& Scalability	& Heuristics	\\ \midrule
  \multirow{5}{*}{{{\bf Bucket}}} 
& Balakrishnan \textit{et al.}~\cite{balakrishnan2006lossless} & Yes		& Blue Gene/L logs	& High	 & Yes \\
& Skibinski \textit{et al.}~\cite{skibinski2007fast}  & Yes		& All logs	& Low	& No	\\
& Hassan \textit{et al.}~\cite{hassan2008industrial} & No		& Telecom logs	& High	& Yes	 \\
& Christensen \textit{et al.}~\cite{christensen2013adaptive}  & Yes		& All logs	& High	& Yes \\
& Feng \textit{et al.}~\cite{feng2016mlc} & Yes		& All logs	& Middle & No \\
\midrule
  \multirow{4}{*}{{{\bf Dictionary}}} 
& Deorowicz \textit{et al.}~\cite{deorowicz2008sub} & No		& Apache web log	& Middle	& Yes \\
& Lin \textit{et al.}~\cite{lin2015cowic} & No	  	& Structured Logs	& High	& Yes	\\
& Mell \textit{et al.}~\cite{mell2014lightweight}  & Yes		& Structured Logs	& High	& No \\
& Racz \textit{et al.}~\cite{racz2004high} & Yes		& Web log 	& High	& Yes	\\
\midrule
  \multirow{3}{*}{{{\bf Statistics}}} 
& Hatonen \textit{et al.}~\cite{hatonen2003comprehensive} & No		& Structured Logs	& High	& Yes\\
& Meinig \textit{et al.}~\cite{meinig2019rough} & No  & All logs & High & Yes \\
& Liu \textit{et al.}~\cite{liu2019logzip} & Yes	& Structured Logs	& Low	& No	\\
\midrule
  \multirow{2}{*}{{{\bf Industry}}} 
& Splunk~\cite{splunk} & Yes	 	& All logs	& Low	& No    \\
& ElasticSearch~\cite{elk} & Yes	& All logs	& Low	& No	\\
\bottomrule
 \end{tabular} 
\end{center}
\vspace{-3pt}
\end{table} 




\subsection{Log Compression Approaches}
\label{sec:log_compress_methods}
According to the techniques employed above, there are three categories of log compression methods: (1) \textit{bucket-based compression} that divides the log data into different blocks and compresses each block in parallel; (2) \textit{dictionary-based compression} that builds a dictionary for fields in the log and replaces strings by referring to the dictionary; and (3) \textit{statistics-based compressors} that apply complex statistical models to find correlations between logs before compression. Note that some log compression methods may involve two or more techniques, in which case we took the major compression technique as their category.

\subsubsection{Bucket-based Compression}
Bucket-based compression methods break the log data into different blocks by some log-specific characteristics and then compresses these blocks in parallel. For instance, many logs show the strong temporal locality or high similarity in certain fields, therefore, these logs can be gathered and then compressed. To tackle the problem that log data were often heterogeneous with varying patterns over time, Christensen \textit{et al.}~\cite{christensen2013adaptive} proposed to partition the log data into different buckets by leveraging the temporal locality and then compress these buckets in parallel. Hassan \textit{et al.}~\cite{hassan2008industrial} adopted a similar idea for telecom logs; however the objective was log event sequence instead of log messages. The log data is firstly broken into equal sized periods and compressed separately. Different from other studies, they use the compressed log event sequences to identify noteworthy usage scenarios for operational profile customization.

Besides, the bucket partition often serves as an initial step towards achieving a high compression ratio. For example, LogPack~\cite{skibinski2007fast} was a multi-tiered log compression method, in which each tier addressed one notion of redundancy. The first tier handled the local redundancy between neighboring lines. The second tier handled the global repetitiveness of tokens while the third tier handled all the remaining redundancy by employing a general compressor. Similarly, Balakrishnan \textit{et al.}~\cite{balakrishnan2006lossless} first observed a number of trends in the Blue Gene/L system logs and proposed several solution to compress the logs accordingly. For example, one trend was that most columns in adjacent logs tended to be the same. At last, the generic compression utilities were applied to further compress the log file.  Hence, they utilized a variant of delta encoding method which compared the log with preceding logs and encoded the differences only. In addition, Multi-level Log Compression (MLC)~\cite{feng2016mlc} divided logs with redundancy into different buckets by calculating the Jaccard similarity among logs. Then, the logs were condensed by a variant of delta encoding, followed by a general compressor to further improve the compression ratio.


\subsubsection{Dictionary-based Compression}
Dictionary-based compression removes the redundancy in log files by replacing repetitive strings with references to a dictionary. For example, some frequent strings (\textit{e.g.}, IP addresses) can be mapped to a condensed string in the dictionary. 
Lin \textit{et al.}~\cite{lin2015cowic} presented a column-wise independent compression for structured logs, which was also very similar to the work presented in~\cite{racz2004high, deorowicz2008sub} though their focuses were web logs. The general idea of these methods is as follows: At first, it splits a log entry into several columns by its fields. After observing  common properties in columns (\textit{e.g.}, common prefixes and suffixes), the method builds a dictionary-based model with Huffman code to compress each column separately. Many general compression techniques can then be applied to achieve a higher compression ratio, including move-to-front coding, phrase sequence substitution, etc. Similarly, Mell \textit{et al.}~\cite{mell2014lightweight} proposed a multi-step method for log compression. It first separated and sorted logs according to particular properties (\textit{e.g.}, value of the first column), and then it created a dictionary where logs are stored by hashing the field name, followed by serializing the dictionary and compressing logs with a general compressor. 


\subsubsection{Statistics-based Compression}
Statistics-based methods realize the log compression by building a statistical model to identify possible redundancy in the log data. Unlike the above two categories of methods which are supported by  manually defined compression logic, the statistics-based compression automatically mines the compression rules. Hatonen \textit{et al.}~\cite{hatonen2003comprehensive} demonstrated a Comprehensive Log Compression (CLC) method to dynamically characterize and combine log data entries. Particularly, the method first identified frequently occurring patterns from dense log data by frequent pattern mining, and then linked patterns to the data as a data directory. 
Meinig \textit{et al.}~\cite{meinig2019rough} proposed an approach adopted from the rough set in the uncertainty theory. It treated the log file as a decision table with removable attributes identified by a one-time analysis of log data. Specifically, attributes that could roughly express each other are then collapsed to one representative attribute. The proposed method belongs to the set of lossy compression approaches which allow the information loss after compression. Lossy compression usually sacrifices the information completeness in raw logs for the high efficiency of log compression. Liu \textit{et al.}~\cite{liu2019logzip} proposed the Logzip method based on log parsing introduced in Section~\ref{sec:log_parsing}. Logzip 
first automatically extracted log templates from raw log messages by a statistical log parsing model. Then Logzip structuralized log templates and other information into intermediate representations, which were finally fed into a general compressor. 

\subsubsection{Others}
Recently, Yao \textit{et al.}~\cite{yaostudy} provided an empirical study on comparing the performance of general compressors on compressing log data against natural language data. Although the study was targeted on general compressors instead of specialized log compressors, their findings could potentially guide the design of tailored log compressors. Besides, Otten \textit{et al.}~\cite{otten2008using} presented a systematic review on general compression techniques, based on which they investigated the use of compression for log data reduction and the use of semantic knowledge to improve data compression. Different from the classic log compression, Hamou-Lhadj et al.~\cite{hamou2006summarizing} proposed to summarize the content of logs for the purpose of understanding software system behaviors. In detail, their approach removes implementation details such as utility information from the execution traces by ranking system components under a well-defined metric.


% the figure of comparing logzip and gzip.

% log storage in industrial practice. (web, blog)

% query on compressed log files.




% \rotatebox[origin=c]{90}

 % \item{\textbf{Large volume of data}} Large-scale systems that contain hundreds or even thousands of nodes, provide services to millions of users every day, such as the service systems in Azure and Google. Logs are routinely generated and stored to record important runtime information for problem diagnosis and troubleshooting. However, the great volume of logs makes the log file storage very challenging, for example, logs are generated at a rate of 50 gigabytes per hour~\cite{mi2013toward}. A typical approach to tackle the large scale problem is to use the distributed storage system such as HDFS. Although approachable, the storage cost on the raw logs is very high. Therefore, a log compression method that can effectively reduce the log file size is highly in demand. 
    
    % Long-term storage requirements Many logs require the long-term storage, usually a year or more according to the development life cycle of software products. Historical logs are amenable to discovering fault patterns and identifying recurrent problems [11]. For example, many users often rediscover old problems because they have not installed fix packs [9]. Meanwhile, auditing logs, which record sensitive operations performed by users and administrators, are often required to be kept for at least two years for possible tracking of system misuse in future. Although storage has become much cheaper than before, archiving logs in such a huge volume is still quite costly. It not only takes up a great amount of storage space and electrical power, but also consumes network bandwidth for transmission and replication.
    
    % Semi-structure data format The logs are often of semi-structure format, where some text fields repeatedly occur among different log messages while the other fields are of non-fixed length and dynamically generated. On the one hand, the repeated text strings consume a lot of storage space but do not provide additional information; On the other hand, the semi-structure characteristic of log messages makes it difficult to apply the general file compressor (such as gzip, rar) effectively, which usually performs well on well structured data.

==> [CSUR 2020] Log Survey/sections/log_mining.tex <==
\section{Log Mining}
\label{sec:log_mining}

% Log faithfully reflects the runtime status of system and records significant activities at different critical points, which is of great importance for the monitoring, administering, and troubleshooting of software systems. 
Log mining employs statistics, data mining, and machine learning techniques for automatically exploring and analyzing large volume of log data to glean meaningful patterns and informative trends.  The extracted patterns and knowledge could guide and facilitate monitoring, administering, and troubleshooting of software systems.
In this section, we first elaborate on challenges encountered in log mining (Section~\ref{sec:log_mining_challenges}). Then, we describe the general workflow of log mining (Section~\ref{sec:log_mining_workflow}). Finally, we introduce three major log mining tasks for reliability engineering, including \textit{anomaly detection} (Section~\ref{sec:log_anomaly_detection}), \textit{failure prediction} (Section~\ref{sec:log_failure_prediction}), and \textit{failure diagnosis} (Section~\ref{sec:log_failure_diagnosis}). Other relevant studies with relatively lesser popularity are laid out in Section~\ref{sec:log_mining_others}.


\subsection{Challenges of Log Mining}
\label{sec:log_mining_challenges}

Traditionally, engineers perform simple keyword search (such as "error", "exception", and "failed") to mine suspicious logs that might be associated with software problems, \textit{e.g.}, component failures. Some rule-based tools~\cite{rouillard2004real,prewett2003analyzing,hansen1993automated} have been developed to detect software problems by comparing logs against a set of manually defined rules which describe normal software behaviors. However, due to the ever-increasing volume, variety, and velocity of logs produced by modern software, such approaches fall short for being labor-intensive and error-prone. Moreover, suspicious logs are often overwhelmed by logs generated during software normal executions. Manually sifting through a massive amount of logs to identify failure-relevant ones is like finding a needle in a haystack.

Additionally, inspecting logs for software troubleshooting often requires engineers to possess descent knowledge about the software. However, modern software systems usually consist of many components developed by different engineers, leading to the generation of heterogeneous logs, which makes troubleshooting beyond the ability of a single engineer. Moreover, due to the high complexity of modern software systems, failures could stem from various sources of software and hardware issues. Examples include software bugs, hardware damage, OS crash, service exception, etc. In addition, promptly pinpointing to the root cause by inspecting logs highly relies on engineers' expertise and experience. However, such knowledge is often not well accumulated, organized, and documented. Therefore, sophisticated ways to conduct automatic log mining are in high demand.

% \textbf{Data Quality} A fundamental support for the learning paradigms in machine learning is adequate and high-quality data.

% Meanwhile, little supervised data can be utilized to build machine learning models. Under such circumstances, researchers and practitioners can only resort to unsupervised learning for log analysis. Furthermore, the process of log data annotation is manually done by human experts and hence the generation of anomaly labels is subject to quality variation, so-called noisy labels.

\subsection{A General Workflow of Log Mining}
\label{sec:log_mining_workflow}

The general workflow of log mining is illustrated in Fig.~\ref{fig:lm_workflow}, which mainly consists of four steps, \textit{i.e.}, log partition, feature extraction, model training, and online deployment.

\begin{figure}[t!b]
\centerline{\includegraphics[width=1.0\columnwidth]{figs/log_mining_workflow.pdf}}
\caption{A general workflow of log mining.}
\label{fig:lm_workflow}
\vspace{-5pt}
\end{figure}

% \begin{figure}[t!b]
%     \begin{minipage}{0.49\textwidth}
%         \centerline{\includegraphics[width=1.0\columnwidth]{figs/ad_workflow.pdf}}
%         \caption{Workflow of log anomaly detection}
%         \label{fig:ad_workflow}
%     \end{minipage}\hfill
%       \begin{minipage}{0.49\textwidth}
%         \centerline{\includegraphics[width=1.0\columnwidth]{figs/ad_algorithms.pdf}}
%         \caption{Categories of log anomaly detection algorithms}
%         \label{fig:ad_algorithms}
%     \end{minipage}
% \end{figure}

% \textbf{1) Log parsing}: Raw logs are often unstructured and need to be parsed into structured format before usage. Specifically, log parsing tries to identify the constant/static part and variable/dynamic part of a raw log line. The constant part is commonly referred as log event, log template, or log key (we use them interchangeably hereafter); the variable part stores the value of the corresponding parameters, which could be different depending on specific runs of the system.


\subsubsection{Log Partition}

Modern software systems often adopt a microservice architecture and comprise a large number of modules operating in a multi-threaded environment. Different microservices or modules often aggregate their execution logs into a single log file, which hinders automated log mining. To tackle the problem, interleaved logs should be partitioned into different groups, each of which represents the execution of individual system tasks. The partitioned log group is the basic unit in extracting features before constructing log mining models. Moreover, studies~\cite{he2016experience} show that the way to partition logs impacts the log mining performance. In the literature, we observe that two elements often serve as the log partitioner, namely, \textit{timestamp} and \textit{log identifier}.

\textbf{Timestamp}. It records the occurrence time of each log, which is a fundamental feature supported by many logging libraries, such as Log4j. Through regexs, the timestamp with different formats can be easily extracted from raw logs in log parsing phase (Section~\ref{sec:log_parsing}).
% To partition logs based on timestamp, logs should guarantee to be sorted chronologically.
In general, two strategies are often adopted to conduct timestamp-based log partition, \textit{i.e.}, fixed window and sliding window. Fixed window has a predefined window size, which means the time span or time interval (\textit{e.g.}, 30 minutes) used to split chronologically sorted logs. Extended from the fixed window, sliding window allows the overlapping between two consecutive fixed windows. The sliding window has two attributes, \textit{i.e.}, window size and step size. The step size indicates the forwarding distance of the window alone the time axis to generate log partitions, which is often smaller than the window size.

% \begin{itemize}
%     \item \textit{Fixed window} has a pre-defined window size, which means the time span or time interval used to split the sorted logs. Particularly, there is no log overlapping between different fixed windows. An example is shown in Fig.~\ref{fig:lm_workflow}, where the window size is $\Delta t$, which could be one hour or one day depending on the specific problem at hand.
    
%     \item \textit{Sliding window} consists of two attributes, \textit{i.e.}, window size and step size. The step size indicates the forwarding distance of the window alone the time axis to generate log partitions. In general, the step size is smaller than the window size, resulting in log overlapping between different sliding windows. Therefore, the strategy of sliding window often produces more log windows than fixed window does, mainly depending on both the window size and step size. In Fig.~\ref{fig:lm_workflow}, the window size is $\Delta t$, while the step size is $\Delta t/3$.
% \end{itemize}

\textbf{Log Identifier}. It is a token identifying a series of related operations or message exchanges of the system. For instance, HDFS logs adopt \textit{block\_id} to record the operations (\textit{e.g.}, allocation, replication, and deletion) on a specific block. Common log identifiers include \textit{user ID}, \textit{task/session/job ID}, \textit{variable/component name}, etc., which can be extracted by log parsing. Compared to timestamp, log identifier is a clearer and more definite signal for partitioning logs. Therefore, many research studies~\cite{qfu09} employed the log identifier for its ability in distinguishing logs of different task executions.
% \textcolor{red}{This is because distributed systems have the problem of clock synchronization, which may produce logs}
However, the log identifiers might be non-unique in representing distinct system entities in different logs, such as virtual machines, physical machines, and networks~\cite{yu2016cloudseer}. This is because, for example, identifiers may not be propagated and synchronized across different services, one thread or process may serve more than one request through multiplexing, etc. Therefore, dedicated algorithms have been developed to address this problem and we elaborate on them later.

\subsubsection{Feature Extraction}
To analyze logs automatically, textual logs in a log partition should be transformed into appropriate formats that could fit machine learning algorithms. Through reviewing the literature, we identified two categories of log-based features, namely, numerical feature and graphical feature. Particularly, numerical feature is the mainstreaming feature which is widely used in the log analysis community.

\textbf{Numerical Feature}. It represents log's statistical properties including numerical and categorical fields that can be directly extracted from logs. It conveys the information of a log partition into a numerical vector representation. Particularly, numerical features employed by most of the existing work are similar and share some typical forms. In the following, we compactly summarize four types of such features.

% In particular, the first three feature types can be automatically obtained by log parsing; while the last one requires some domain knowledge to identify relevant and representative features based on the software system and problem context.

% \textbf{Numerical feature} represents log's statistical properties including numerical and categorical fields that can be directly extracted from logs. It conveys the information of individual logs and pays less attention to their interactions. We summarize the following four types of features, which are employed by most of the existing work. Each feature vector corresponds to one group of partitioned logs in the previous step. In particular, the first three types of features can be automatically obtained through straightforward log data pre-processing; while the last one requires some domain knowledge to identify relevant and representative features based on the context of the problem.

% feature vector construction (log vectorization), \textit{e.g.}, log sequences

\begin{itemize}
	\item \textit{Log event sequence}: A sequence of log events recording system's activities. Particularly, each element can simply be the log event ID or log embedding vector, \textit{e.g.}, learned by word2vec algorithms~\cite{mikolov2013distributed}.
	
	\item \textit{Log event count vector}: A feature vector recording the log events occurrence in a log partition, where each feature denotes a log event type and the value counts the number of occurrence.
	
	\item \textit{Parameter value vector}: A vector recording the value of parameters (\textit{i.e.}, variables extracted by log parsing) that appear in logs.
	
	\item \textit{Ad-hoc features}: A set of relevant and representative features extracted from logs, which are defined using domain knowledge on the object software system and problem context. For example, Zhou \textit{et al.}~\cite{zhou2019latent} manually identified various types of features from system trace logs, including configuration (\textit{e.g.}, memory limit, CPU limit), resource (\textit{e.g.}, memory consumption, CPU consumption), etc. These features profile the typical health states of a system.
\end{itemize}


\textbf{Graphical Feature}. To discover the hierarchical and sequential relations (\textit{e.g.}, dependency and co-occurrence) between system components and events with logs, the graphical feature usually produces a directed graph model characterizing system behaviors, \textit{e.g.}, the execution path of a process.
% In workflow graph, each node stands for a log event, \textit{i.e.}, a log template, and the edge represents the transition from one log event to another.
% Unlike numerical features, graphical feature focuses on the relationships between logs (\textit{e.g.}, dependency and co-occurrence), thus describes complete functionalities of the system. 
The graphical features serve as the foundation for a variety of downstream log mining tasks (such as monitoring~\cite{zhao2016non,yu2016cloudseer} and diagnosis~\cite{nandi2016anomaly,amar2018using,bao2019statistical}). For example, log-based behavioral differencing~\cite{goldstein2017experience} can identify system executions that are derived from system normal behaviors, which has various applications in system evolution, testing, and security~\cite{bao2019statistical}.
% \textcolor{red}{One challenge for graph construction is that there could be concurrently running threads/tasks in the system, producing interleaved logs.}
In this section, we briefly introduce the algorithms used by existing work for graphical feature extraction, which can be roughly categorized into two lines of work.

The first line of work leverages the objects identified in logs, \textit{e.g.}, process ID and system component name, to construct graphs for system state monitoring. As objects often demonstrate complicated hierarchical relations, it usually needs a more sophisticated algorithm for log partition. For instance, to represent execution structure and object hierarchy in logs, Zhao \textit{et al.}~\cite{zhao2016non} constructed a stack structure graph by considering the 1:1, 1:n, and n:m mappings among different objects. 
% Yu \textit{et al.}~\cite{yu2016cloudseer} employed task- or thread-related identifiers to group related logs. However, as unique identifiers are often unavailable, they proposed to group interleaved logs which share a common set of identifiers. Finally, each log containing an identifier set acts as a state node of the graph, and transitions are added by examining the subset and superset relations of different identifier sets.
To tackle the challenge that unique identifiers are often unavailable, Yu \textit{et al.}~\cite{yu2016cloudseer} proposed to group interleaved logs based on a common set of identifiers. Each log contains an identifier set that acts as a state node of the graph, and transitions are added by examining the subset and superset relations of different identifier sets.
% lou2010mining_b

The other line of work makes use of the underlying statistical distribution of log events, \textit{e.g.}, the order of log events, the temporal and spatial locality of dependent log events, to build various graphs for system behavior analysis. Particularly, some work aims at recovering the exact behavioral model from log traces. Log partition therefore requires that identifiers can tie together the set of events associated with a program execution. For example, Amar \textit{et al.}~\cite{amar2018using} presented two variants of k-Tails~\cite{biermann1972synthesis}, namely 2KDiff and nKDiff, to build Finite State Machine (FSM) for log differencing. 2KDiff computes and highlights the differences between two log files containing a set of partitioned logs; while nKDiff is able to conduct the comparison for multiple log files at once. Later Bao \textit{et al.}~\cite{bao2019statistical} extended their work by proposing s2KDiff and snKDiff, which take into consideration the frequencies of different behaviors. Busany \textit{et al.}~\cite{busany2016behavioral} studied the scalability problem of existing behavioral log analysis algorithms by extracting Finite State Automaton (FSA) models or temporal properties from logs. We refer readers to this paper for more related studies.
% Particularly, they suggested to analyze only a sample of log traces and provided statistical guarantees to support the correctness of the analysis result. 

However, as previously discussed, a unique identifier for each execution trace is not always available, especially in distributed applications and systems. Therefore, some work attempts to mine behavioral models using interleaved logs. For example, Lou \textit{et al.}~\cite{lou2010mining_b} employed statistical inference to learn the temporal dependencies among log events, which is also studied in similar work including~\cite{beschastnikh2014inferring,beschastnikh2011leveraging}. Nandi \textit{et al.}~\cite{nandi2016anomaly} computed the nearest neighbor groups to capture the temporal co-occurrence of log events more accurately. The resulted model is a program Control Flow Graph (CFG) spanning distributed components. Particularly, the correlation between two components is calculated using either the Jaccard similarity or the Bayesian conditional probability approach. Du \textit{et al.}~\cite{du2017deeplog} described two methods to capture service executions by FSA models. The first method leverages the trained log anomaly detection model, whose predictions encode the underlying path of task execution. The second method builds a matrix where each entry represents the co-occurrence probability of two log keys appearing together within a predefined distance.

% described Stitch, a non-intrusive tool that can profile the performance of an entire distributed software stack. Specifically, they built a system stack structure graph, whose nodes contain respective log messages arranged chronologically. Debugging can then be conducted by monitoring the status of different system objects. To construct the graph, they extracted from raw logs the object identifiers and their types, which are associated based on their co-occurrences in log messages. An algorithm is proposed to identify the execution structure and hierarchy between objects, which is a directed acyclic graph. Logs containing correlated objects are put in the same node of the structure graph.


% Pi \textit{et al.}~\cite{pi2018profiling} proposed LRTrace, a tracing and feedback control tool for profiling distributed applications in a non-intrusive manner. Such tool can facilitate the understanding and troubleshooting of cloud distributed systems. To this end, they defined a set of regular expressions to identify different entities in a log, \textit{e.g.}, task ID, parameter type and value, etc. Logs and resource metrics that share identical ID fields, namely, application ID and container ID, are matched together. Taking advantage of such design, operations such as \textit{Groupby}, \textit{Count}, and \textit{Sum} can be easily applied for data analytical jobs in different granularities, \textit{e.g.}, the CPU usage of a certain task in a certain container. Failures and performance issues can then be detected and diagnosed by inspecting system's runtime status.


% In~\cite{du2017deeplog}, Du et al. proposed two methods for mining system workflow. The first method leverages the trained anomaly detection model, whose predictions encode the underlying workflow execution path. The second method builds a co-occurrence matrix where each entry represents the probability of two log keys appearing within a predefined distance in log sequences. Such matrix can be used to calculate the co-occurrence probability of any two log keys, which resembles the concept of \textit{Confidence} in association rule learning. Logs with co-occurrence probability larger than a threshold will be linked together. Nandi \textit{et al.}~\cite{nandi2016anomaly} also considered the temporal co-occurrence of log templates to mine program \textcolor{red}{CFG}. Specifically, they compute Nearest Neighbor Groups (NNGs) for each log template to prune away noise due to the interleaving of threads, which are used to mine only immediate predecessors/successors of a template. Three types of CFG's sub-structures are considered when computing NNGs, namely, linear sequences, forks, and merges. Yu \textit{et al.}~\cite{yu2016cloudseer} constructed the workflow model by leveraging task- or thread-related identifiers in logs. However, as unique identifiers are often unavailable, they proposed to group logs which share a set of identifiers. Chothia \textit{et al.}~\cite{chothia2017online} proposed an approach to reconstruct user sessions, communication dependencies, and trace tree clusters online. This is done by combining the correlators with other fields present in the logs. Specifically, they expressed the needed computations in data-parallel fashion using a dataflow model, which can be executed efficiently using Timely Dataflow.

% lprof~\cite{zhao2014lprof}


\subsubsection{Model Training}

In this process, appropriate algorithms are selected based on the problem at hand and selected models are trained based on the extracted features. A variety of machine learning algorithms have been proposed, and we leave more details in the following sections. This step is often conducted in an offline manner.
Moreover, a fundamental assumption of various log mining tasks is that the majority of logs should exhibit patterns that conform to system's normal behaviors. For example, in anomaly detection, different models are trained to capture various patterns from different perspectives and used to detect anomalies that lack the desireable properties. 

\subsubsection{Online Deployment}

Once the model is trained offline, it could be deployed to real-world software systems for various log mining tasks. For example, an anomaly detection model can be integrated into software products to detect malicious system behaviors and raise alarms in real time. To tackle the challenge of pattern change caused by system upgrades, several studies~\cite{du2017deeplog,lin2016log} supported online update of a previously trained model to adapt to unprecedented log patterns.

% could lead to 
% Since  in their product life cycle, a previously trained model may not fit the pattern changes.
\begin{figure}[t!b]
\centerline{\includegraphics[width=0.6\textwidth]{figs/ad_algorithms.pdf}}
\caption{A taxonomy of log anomaly detection algorithms.}
\label{fig:ad_algorithms}
\vspace{-5pt}
\end{figure}

\subsection{Anomaly Detection}
\label{sec:log_anomaly_detection}
\subsubsection{Problem Formulation} Anomaly detection is the task of identifying system anomalous patterns that do not conform to expected behaviors on log data. Typical anomalies often indicate possible error, fault or failure in software systems. In this section, we elaborate on existing research work in this field based on approaches adopted therein. As shown in Fig.~\ref{fig:ad_algorithms}, we categorize the approaches into two broad classes: traditional machine learning algorithms and deep learning models. The surveyed approaches are listed in Table~\ref{tab:anomaly_detection_summary} together with several interesting properties. Specifically, we summarize the algorithm/model and feature used by an approach and whether or not each approach is unsupervised and online. Particularly, unsupervised approaches do not require labels for model training; and an online approach is one that can process its input piece-by-piece in a streaming fashion. In this paper, we mainly focus on general types of anomalies that are natural imperfections of software systems and will directly impact system's reliability. External attacks and intrusions (such as cyber attacks and malicious activities) that are more relevant to system's security go out of the scope for this paper.

% A reference: incremental analysis of large-scale system logs for anomaly detection

\begin{table}[t]
\begin{center}
\caption{Summary of log anomaly detection approaches.}
\label{tab:anomaly_detection_summary}
 \begin{tabular}{c|c|c|c|c|c}
  \toprule
\multicolumn{2}{c|}{\bf Methods} & Algorithm/Model & Feature & Unsupervised & Online \\
\midrule
  \multirow{13}{*}{\rotatebox[origin=c]{90}{{\textbf{Traditional machine learning}}}} 
& Xu \textit{et al.}~\cite{xu2009detecting} & PCA & $\star$~$\dagger$ & Yes & No \\
& Lin \textit{et al.}~\cite{lin2016log} & Clustering & $\ast$ & Yes & No \\
& He \textit{et al.}~\cite{he2018identifying} & Clustering & $\ast$~$\star$ & Yes & No \\
& Liang \textit{et al.}~\cite{liang2007failure} & SVM & $\ddagger$ & No & No \\
& Kimura \textit{et al.}~\cite{kimura2018proactive} & SVM & $\ddagger$ & No & No \\
& Xu \textit{et al.}~\cite{xu2009online} & Frequent pattern mining & $\ast$~$\star$ & Yes & Yes \\
& Shang \textit{et al.}~\cite{shang2013assisting} & Frequent pattern mining & $\ast$ & Yes & No \\
& Lou \textit{et al.}~\cite{lou2010mining_a} & Frequent pattern mining & $\star$ & Yes & No \\
& Farshchi \textit{et al.}~\cite{farshchi2015experience} & Frequent pattern mining & $\star$ & Yes & No \\
& Nandi \textit{et al.}~\cite{nandi2016anomaly} & Graph mining & $\P$ & Yes & No \\
& Lou \textit{et al.}~\cite{lou2010mining_b} & Graph mining & $\P$ & Yes & No \\
& Yamanishi \textit{et al.}~\cite{yamanishi2005dynamic} & Statistical model & $\ast$ & Yes & No \\
& He \textit{et al.}~\cite{he2016experience} & Logistic regression & $\star$ & No & No \\

\midrule
  \multirow{6}{*}{\rotatebox[origin=c]{90}{{\textbf{Deep learning}}}} 
& Du \textit{et al.}~\cite{du2017deeplog} & LSTM model & $\ast$~$\dagger$ & Yes & Yes \\
& Zhang \textit{et al.}~\cite{zhang2019robust} & LSTM classification model & $\ast$ & No & No \\
& Meng \textit{et al.}~\cite{meng2019loganomaly} & LSTM model & $\ast$~$\star$ & Yes & Yes \\
& Xia \textit{et al.}~\cite{xia2020loggan} & LSTM-based GAN model & $\ast$ & Yes & Yes \\
& Lu \textit{et al.}~\cite{lu2018detecting} & CNN model & $\ast$ & No & No \\
& Liu \textit{et al.}~\cite{liu2019log2vec} & Graph embedding model & $\P$ & Yes & No \\
\midrule

\multicolumn{6}{l}{$\ast$~Log event sequence, $\star$~Log event count vector, $\dagger$~Parameter value vector} \\
\multicolumn{6}{l}{$\ddagger$~Ad hoc features, $\P$~Graphical feature}\\
\bottomrule
 \end{tabular} 
\end{center}
\vspace{-4pt}
\end{table}


\subsubsection{Traditional Machine Learning Algorithms}

Traditional machine learning algorithms usually perform on top of features explicitly provided by practitioners, \textit{e.g.}, log event count vector. Particularly, the anomaly detection task can be formalized into different types and solved with different algorithms such as clustering, classification, regression, etc.
%  Therefore, feature engineering is a critical step. 

\textbf{Dimensionality Reduction}. It transforms data of high dimension into a low-dimension representation such that some meaningful properties of the original data can be retained in the low-dimension space. Principal Components Analysis (PCA) is one of the most popular algorithms of this kind. By projecting data points to the first \textit{k} principal components, anomalies can be identified if the projected distance is larger than a threshold. 
% To extract log template accurately, they proposed a statistic code analysis approach which executes directly on the source code or binary code. Specifically, they first parsed source code into Abstract Syntax Tree (AST) and then expanded all \textit{toString()} calls in each logging statement to retrieve the complete message template. The underlying assumption is that the source code is available, which may not always hold in practical scenarios.
PCA was first applied by Xu \textit{et al.}~\cite{xu2009detecting,xu2009online} to mine system problems from console logs. Particularly, both log event count vector and parameter value vector are constructed and fed into a PCA model for anomaly detection.
% \textcolor{red}{In~\cite{gurumdimma2016crude}, Gurumdimma et al. proposed an approach to detect errors in  large-scale distributed systems. Specifically, they calculate the Mutual Information and Entropy for log sequences within a time window. The essential idea is that log sequences that exhibit higher uncertainty are more likely to signify abnormal system behaviours. As a complement, they identify a list of 96 elements of resource usage data, \textit{e.g.}, read bytes, write bytes etc., and apply PCA for outlierness checking.}

\textbf{Clustering}. As an unsupervised method, clustering-based anomaly detection groups log-based feature vectors into different clusters such that vectors in the same cluster are more similar to each other (and as dissimilar as possible to vectors from other clusters). Clusters that contain very few data instances tend to be anomalous. For example, Lin \textit{et al.}~\cite{lin2016log} proposed LogCluster, which clusters log sequences and recommends a representative sequence to assist developers quickly identify potential problems. The representative sequence is selected by calculating the cluster centroid.
% Particularly, they used Inverse Document Frequency (IDF)-based and contrast-based event weightings to calculate the discriminative power of different log events for problem identification. The contrast-based event weighting masks log events which appear both in lab and production environments.
Furthermore, He \textit{et al.}~\cite{he2018identifying} proposed the Log3C framework to incorporate system KPIs into the identification of impactful problems in service systems. In particular, they proposed a cascading clustering algorithm to group numerous log sequences promptly. They finally use a multivariate linear regression model to identify impactful problems that lead to KPI degradation.
% Similarly, they used two types of log event weightings, namely, IDF and importance weightings, where the latter is done by fitting a linear regression model between log events and system KPIs. 

% Specifically, they first sample a portion of log sequences and cluster them using HAC algorithm. For each cluster, the mean vector of all the sequence vectors is calculated to be the representative vector. The unsampled log vectors will be assigned by examining the similarity with the representative vector of each cluster.

% Many works involve a process of manual feature selection~\cite{makanju2012spatio,liu2018integrated}. For example, Makanju \textit{et al.}~\cite{makanju2012spatio} proposed Spatio-Temporal Alert Detection (STAD), a framework to detect alerts by analyzing system logs which are partitioned temporally and spatially. Specifically, they first summarized alerts' properties and then developed dedicated rules to cluster system logs. In~\cite{liu2018integrated}, Liu et al. first identified ten features relating to user behaviors. Then, a K-prototype clustering algorithm is applied to cluster system logs. The clusters which are obviously benign will be filtered out first. Finally, a k-NN classifier is used to generate accurate detection results.

% \textbf{Tree} \textcolor{red}{Tree based [17], [18] (decision tree), both are for failure diagnosis instead of anomaly detection}

\textbf{Classification}. Anomaly detection with classification categorizes the log partition into either normal or anomalous type, where anomalous examples are derived from normal ones in terms of some statistical properties. Support Vector Machine (SVM) is a supervised classification method that is commonly used for log anomaly detection. In~\cite{liang2007failure}, Liang et al. vectorized log partitions by identifying six types of features, including events number in a time window, accumulated events number, etc. Based on these features, they applied four classification models for anomaly detection, \textit{i.e.} including SVM and nearest neighbor predictor. In addition, Kimura et al.~\cite{kimura2018proactive} proposed a log analysis method for proactive failure detection based on logs' characteristics, including frequency, periodicity, burstiness, and correlation with maintenance and failures. A SVM model with the Gaussian kernel is employed for detecting failures.

\textbf{Frequent Pattern Mining}. It aims to discover the most frequent item sets and sub-sequences in a log dataset that characterize system's normal behaviors. Data instances that do not conform to the frequent patterns will be reported as anomalies. The presence of specific log events and the order of log events can both constitute patterns. For example, Xu \textit{et al.}~\cite{xu2009online} mined sets of log messages that often co-occur to detect abnormal execution traces in an online setting. Compared to offline approaches, online pattern matching can quickly identify benign system executions, thus striking a balance between accuracy and efficiency.
Similarly, Lim \textit{et al.}~\cite{lim2008log} searched for item sets that were commonly associated with different failure types. Such item sets can assist developers in predicting and characterizing failures.
Other approaches mine the sequential patterns by log events to discover anomalies or bugs~\cite{shang2013assisting,lu2018cloudraid}.
% Shang \textit{et al.}~\cite{shang2013assisting} proposed an approach to assist developers in maintaining big data analytics applications such as Hadoop. They examined the differences between execution log sequences produced in lab and in production environments.
% In particular, to recover sequences of the execution logs, they first linked abstracted log events with task ids, and then simplified sequences by removing redundant log events.

% Debnath \textit{et al.}~\cite{debnath2018loglens} proposed an approach to automatically learn log patterns from systems normal runs for anomaly detection, called LogLens. Specifically, LogLens first clusters logs using LogMine algorithm. For all logs within a same cluster, various fields and entities will be identified to constitute the unique patterns of that cluster, \textit{e.g.}, ip, action, username, etc. Then, LogLens uses the discovered patterns to parse logs. Logs that fail to match with any patterns will be reported as anomalies. Moreover, logs with a same id field with be grouped into sequences to build a Finite State Automaton (FSA)-based model, which encodes log sequences produced by normal system events. Log sequences that exhibit anomalous behaviors can be automatically identified.

Additionally, Lou et al. ~\cite{lou2010mining_a} were the first to consider mining invariants among log messages for system anomaly detection.
% Specifically, they first parsed raw logs and grouped them according to log parameters.
Two kinds of invariants that model the relations between the number of different log messages are derived: (1) invariants in textual logs that describe the equivalence relation; and (2) invariants as a linear equation, which is the linear independence relation. Farshchi \textit{et al.}~\cite{farshchi2015experience} proposed a similar approach which mines the correlation and causation relations between log events and cloud system metric changes. Specifically, they employed a regression-based approach to learn a set of assertions modeling the linear relations. Anomaly detection is then conducted by monitoring log event streams and checking the compliance of metrics against the assertions.

\textbf{Graph Mining}. The set of approaches mainly employs graphical features, \textit{i.e.}, various graph models (Section~\ref{sec:log_mining_workflow}), to identify behavioral changes of complex systems, which can be used for early detection of anomalies and allowing proactive actions for correction. For example, Nandi \textit{et al.}~\cite{nandi2016anomaly} introduced a CFG mining approach to detect anomalous runtime behaviors of distributed applications from execution logs, including both sequence anomaly and distribution anomaly. A sequence anomaly is raised when an expected child is missing for a parent node within the given time interval; a distribution anomaly is raised when an edge probability is violated. In~\cite{qfu09}, Fu et al. modeled the execution behaviors of each system module as a state transition graph by learning an FSA from log sequences. 
Each transition in the learned FSAs corresponds to a log key. For each state transition, two types of information (\textit{i.e.}, the time consumed and circulation number) are recorded and applied to detect two performance issues: low transition time and low transition loop. By employing the Gaussian distribution to model the state transition in a distributed system,  low-performance transitions can be automatically identified by setting a proper threshold.
% Specifically, for each state transition in FSA, the time (or circulation number) recorded in all machines of a distributed system are fitted with a Gaussian distribution. By setting a threshold, the transitions with low performance can be automatically identified.

\textbf{Other Statistical Models}. There are some algorithms that do not belong to the above categories. For example, Yamanishi \textit{et al.}~\cite{yamanishi2005dynamic} employed a mixture of Hidden Markov Models to monitor syslog behaviors. Particularly, the model is learned with an online discounting learning algorithm by dynamically selecting an optimal number of mixture components. Anomaly scores are assigned using universal test statistics whose threshold can be dynamically optimized.
He \textit{et al.}~\cite{he2016experience} employed a logistic regression model to detect anomalies. They adopted event count vectors as the feature and trained the model with a set of labeled data. A testing instance is declared as anomalous when the probability estimated by the logistic function is greater than 0.5.
Nagaraj \textit{et al.}~\cite{nagaraj2012structured} diagnosed performance issues for large-scale distributed systems by finding a set of inter-related log event occurrences and variable values that exhibit the largest divergence across logs sets. Specifically, they first separated logs into two sets according to some performance metrics (\textit{e.g.}, runtime). Then, they recommended log events or state variables that contribute the most to the performance difference via t-tests.


\subsubsection{Deep learning models} Deep learning uses a  multiple-layer architecture (\textit{i.e.}, neural networks) to progressively extract features from inputs with different layers addressing different levels of feature abstraction. Due to the exceptional ability in modeling complex relationships, neural networks are widely applied in log-based anomaly detection. In the literature, we observed a significant portion of papers adopting the Recurrent Neural Network (RNN) model and its variants. Hence, we classify the deep learning  models into RNN-based models and other models.

% \textbf{LSTM-based models}. Zhang \textit{et al.}~\cite{zhang2016automated}, to the best of our knowledge, are the first to exploit LSTM model on log data for system failure prediction, which paved the path for more applications of LSTM model on log analysis. For example, 


\textbf{RNN-based Models}. Models belonging to the RNN family (such as LSTM model and GRU model) are commonly used to automatically learn the sequential patterns in log data. Anomalies are raised when log patterns deviate from the model's predictions. For example, Du \textit{et al.}~\cite{du2017deeplog} proposed DeepLog, which utilizes an LSTM model to learn system's normal execution patterns by predicting the next log event given a sequence of preceding log events. However, some anomalies may manifest themselves as an irregular parameter value instead of a deviation from a normal execution path. Hence, DeepLog also applies an LSTM model for checking the validity of parameter value vectors.
% \textcolor{red}{Yen et al. adopted similar settings in their work~\cite{yen2019causalconvlstm}. However, they further utilized Convolutional  Network Network (CNN)'s efficiency of spatial feature extraction and proposed a hybrid model called CasualConvLSTM. Meanwhile, to deal with concept drift. They closely monitored model's false positive count/rate. When they exceed a pre-defined threshold, model retraining will be triggered.}
% have a closed-world hypothesis, which 
Many existing studies assume that the log data are stable over time and the set of distinct log events is fixed and known. However, Zhang \textit{et al.}~\cite{zhang2019robust} found that log data often contain previously unseen log events or log sequences, demonstrating log instability.
% Particularly, such instability results from the evolution of logging statements and the processing noise in log data.
To tackle this problem, they proposed LogRobust to extract the semantic information of log events by leveraging off-the-shelf word vectors and then applied a bidirectional LSTM model to detect anomalies.
% During log vectorization, TF-IDF is applied to identify the weight of different log tokens.

In terms of capturing log's semantics, Meng \textit{et al.}~\cite{meng2019loganomaly} found existing word2vec models did not distinguish well between synonyms and antonyms. Therefore, they trained a word embedding model to explicitly consider the information of synonyms and antonyms. Meng \textit{et al.}~\cite{mengsemantic} further extended their work by proposing a semantic-aware representation framework for online log analysis. The issues of log-specific word embedding and out-of-vocabulary (OOV) are both addressed.
% Besides log sequential patterns, they also calculate log event count vectors as quantitative patterns. LSTM model is applied upon these two patterns for anomaly detection.
% Experiments on log classification and anomaly detection demonstrate the contribution of log semantic understanding to the analysis of logs.
Recently, Zuo \textit{et al.}~\cite{zuo2020intelligent} combined the transaction-level topic modeling for learning the embedding of logs, where a transaction is a group of logs sequentially occurring in a time window. To address the problem of insufficient labels, Chen \textit{et al.}~\cite{chen2020cross} applied transfer learning to share anomalous knowledge between two software systems. Specifically, they first trained an LSTM model on the data with sufficient anomaly labels to extract sequential log features, which were then fed into fully connected layers for anomaly classification. Next, the LSTM model was fine-tuned with logs from another system with limited labels, while the fully connected layers were fixed.
% In this process, the  fully connected layers are fixed to ensure knowledge is transferred.

\textbf{Other Deep Learning Models}. Besides the RNN-based models, other model architectures also play a role in detecting anomalies with logs. For example, 
% Borghesi \textit{et al.}~\cite{borghesi2019anomaly} used autoencoders to detect anomalies in supercomputers. Specifically, for each node, an autoencoder is trained to characterize its normal behaviors, \textit{i.e.}, a set of measurements. Anomaly is raised when the reconstruction error calculated by the model is large, \textit{i.e.}, it cannot correctly reconstruct the input.
Xia \textit{et al.}~\cite{xia2020loggan} proposed LogGAN, an LSTM-based Generative Adversarial Network (GAN). Like all GAN-style models, LogGAN comprises a generator and a discriminator. The generator attempts to capture the distribution of real training data and synthesizes plausible examples;
% , which is a fake training dataset consisting of both normal and abnormal logs; 
while the discriminator tries to distinguish fake instances from real and synthetic data. 
% Finally, the trained generator is applied for anomaly detection for upcoming logs.
Effort is also devoted to explore the feasibility of Convolutional Neural Networks (CNN) for anomaly detection. Specifically, Lu \textit{et al.}~\cite{lu2018detecting} first utilized a word embedding technique to encode logs into two-dimension feature matrices, upon which CNN models with different filters were then applied for anomaly detection. Liu \textit{et al.}~\cite{liu2019log2vec} proposed log2vec, a graph embedding based method for cyber threat detection. Specifically, they first converted logs into a heterogeneous graph using heuristic rules and then learned the embedding of each log entry by a graph representation learning approach. Based on the embedding vectors, logs were grouped into clusters, whose size smaller than a threshold would be reported as malicious.
% , such as connecting the logs of the same user.

% \textcolor{red}{LSTM models have been criticized for being black-box when making predictions, which has hindered their applications in critical system decision stages. Brown \textit{et al.}~\cite{brown2018recurrent} tried to bridge this gap by improving models' interpretability with a series of attention mechanisms. Experiments show their approaches can help explain the predictions produced by different LSTM models. Besides LSTM model and its variants, other types of deep learning models are also exploited.}

% To address the problem of insufficient labels, XXX et al.[xxx] applied transfer learning to share anomalous knowledge between two software systems. Specifically, they first train a LSTM model on data with sufficient anomaly labels to extract sequential features of logs, which are then fed into fully connected layers for anomaly classification. Next, the trained LSTM model is fine tuned with logs from another system, who often has limited labels. In this process, the fully connected layers are fixed to make sure knowledge is transferred.

% In~\cite{cui2018convolutional}, Cui et al. observed that in many traditional machine learning methods, the vector representation of log events ignores their temporal patterns. Therefore, they proposed to divide each time window of logs into sequential subwindows and construct a 2D matrix to capture logs' temporal dependencies. A multi-module convolutional auto-encoder is then used to extract log features, which are fed into a SVM for classification. Farzad \textit{et al.}~\cite{farzad2020unsupervised} used two Autoencoders combined with Isolation Forest model for anomaly detection. The first Autoencoder is used to extract features, which are fed into the Isolation Forest model for positive sample prediction. A small portion of positively predicted samples are used for training another Autoencoder, which extracts features for the remaining samples. Finally, anomalies are detected by computing a threshold.

\subsection{Failure Prediction}
\label{sec:log_failure_prediction}
\subsubsection{Problem Formulation}
% From the collection of normal logs, 
Anomaly detection aims to detect anomalous status or unexpected behavior patterns which may or may not cause failures. Differently, failure prediction attempts to proactively generate early warnings to prevent server failures, which often lead to unrecoverable states.
The objective and role of anomaly detection and failure prediction are different yet both are important. 
Therefore, the exploration of failure prediction techniques is significant to reliability engineering.
Generally, when software systems deviate from fulfilling a required system  function~\cite{laprie1995dependable}, a failure occurs and it often shows human-perceivable symptoms. The failure could lead to unintended results and user dissatisfaction, especially for large-scale software systems. Traditional ways of failure management (such as anomaly detection) are mostly passive, which deal with failures after they have happened. In contrast, failure prediction aims to proactively predict the failure before it happens. A common practice is to leverage the valuable logs to proactively predict failures. For example, in~\cite{zhang2018prefix}, switch failures in data center networks are predicted from current status and curated historical hardware failure cases. Usually, input data of the predictive model are system logs, which record the system status, changes in configuration, and operational maintenance, etc.

% In cloud systems, failure is considered as a different scenario that an event occurs when the delivered service deviates from correct service.

% However, more valuable way to handle failure is to proactively predict failures so that maintainer can intervene and fix the problem before it become to a failure.

% motivations
% Failures occurred in software systems could degrade user experience and further mitigate system performance.
%In many software companies, despite enormous efforts spent on software quality engineering, countless types of failures occur in software systems in daily operations.

% significant of solving this problem
% Currently, the main-stream DevOps policy accelerates the repetition of development and maintenance tasks.
% Developers continuously polish existing features, implement new features, and release new versions within a short time to address the requirements of changing market.
% When customers encounter a problem, they often describe their situation and submit a simple report with limited instructive information to the technical support team of the software system.
% For a popular software system, the support team needs to collect and analyze a large number of issue or bug reports from customers to guide the system maintenance.
% Therefore, how to manage failures efficiently is a huge challenge both for support team and DevOps engineers.

% management of failure via event logs


% different settings
According to the source of failures, failure prediction could mainly be categorized into two scenarios: 
a) Prediction of independent failures in homogeneous systems, \textit{e.g.}, high-performance computing (HPC) systems.
Most existing approaches focus on how to leverage the sequential information to predict the failure of each single component, \textit{i.e.}, sequence-based methods.
b) Prediction of outages caused by a collection of heterogeneous devices or components, which is widely observed in large-scale cloud systems.
The mainstreaming approach tends to explore useful hints in the relationship between multiple heterogeneous components and makes prediction from relation-mining algorithms.
%\textcolor{red}{why methods used in different systems are different? should explain more details about the disparate points}
% % motivations
% Failures occurred in software systems could degrade user experience and further mitigate system performance.
% In many software companies, despite enormous efforts spent on software quality engineering, countless types of failures occur in software systems in daily operations.
% In cloud systems, failure is considered as a different scenario that an event occurs when the delivered service deviates from correct service.
% % significant of solving this problem
% Currently, the main-stream DevOps policy accelerates the repetition of development and maintenance tasks.
% Developers continuously polish existing features, implement new features, and release new versions within a short time to address the requirements of changing market.
% When customers encounter a problem, they often describe their situation and submit a simple report with limited instructive information to the technical support team of the software system.
% For a popular software system, the support team needs to collect and analyze a large number of issue or bug reports from customers to guide the system maintenance.
% Therefore, how to manage failures efficiently is a huge challenge both for support team and DevOps engineers.

% % management of failure via event logs
% Traditional failure management for software systems deals with failures after they have happened.
% However, more valuable way to handle failure is to proactively predict failures so that maintainer can intervene and fix the problem before it become to a failure.
% For example, in~\cite{zhang2018prefix}, switch failures in data center networks are predicted from current status and curated historical hardware failure cases.
% Usually, input data of the predictive model are system event logs, such as system status, changes in configuration, and operational maintenance.
% Hence, proactive failure prediction should be conducted by analyzing system logs.
% % different settings
% According to the source of failures, proactive failure prediction is categorized into two scenarios: 
% a) Prediction of independent failures in homogeneous devices. 
% The typical circumstance comes from the cluster of high-performance computing system.
% b) Prediction of outage caused by a collection of heterogeneous devices.  
% It is more important in large-scale cloud systems.

%\subsubsection{Sequence-based Methods}
\subsubsection{Homogeneous Systems} In homogeneous systems, the mainstreaming approaches are based on modeling the sequential information that represents the system status.
A typical homogeneous system is large-scale supercomputers which may encounter faults (e.g., component failures) every day.
Exascale systems are expected to combat with higher fault rates due to enormous number of system components and higher workload~\cite{das2018desh}.
% Motivation
However, triggering resilience-mitigating mechanisms is difficult since there are no obvious, well-defined failure indicators, which rely on a deeper understanding of the faults caused by hardware and software components.
Therefore, logs become the most reliable information source to monitor the system health.
% Generation of proactive alert
Furthermore, to catch early warning signs of these failures, there are additional applications that scan through the monitoring data from the system logs and proactively generate alerts.
Some of these alerts are generated from the manually defined thresholds on the collected system performance data (\textit{e.g.}, CPU utilization rate) or error logs (\textit{e.g.}, certain types of errors appearing too frequently within some time range).
The objective of such alerts is to provide early warnings so that protective actions (\textit{e.g.}, virtual machine migration or software rejuvenation) can be performed to mitigate or minimize the impact of such failures.
In this context, efficient failure prediction via system log mining can enable proactive recovery mechanisms to increase reliability.

% methods
In homogeneous systems, component failures or node soft lock-ups typically lead to crashes of user jobs scheduled on the affected nodes, and they may cause undesired downtime.
One approach to mitigate such problems is to predict node failures with a sufficient lead time in order to take proactive measures.
Sahoo \textit{et al.}~\cite{sahoo2003critical} first addressed this problem by collecting system logs representing the components' health status. Then, several time series models are employed to predict the system health of each node through indication metrics, such as the percentage of system utilization, usage of network IO, and system idle time.
% add new citation
Russo \textit{et al.}~\cite{russo2015mining} considered the log sequence as multi-dimensional vector and employed three kinds of support vector machines to predict defective log sequences.
% log events representing the failure chain
% RNN-based methods
Das \textit{et al.}~\cite{das2018desh} proposed Desh to identify failure indicators in each node with enhanced training and classification for failure event log chain. Desh is a deep learning-based method that contains three phases:
(1) It first recognizes chains of log events leading to a failure. 
(2) Then it re-trains chain recognition of events augmented with expected lead times to failure; 
(3) Finally Desh predicts lead times during testing/inference deployment to predict which specific node fails in how many minutes.
% online learning methods
To speed up the recognition of the failure chain from log events, Das \textit{et al.}~\cite{das2020aarohi} proposed a new node failure predicting method called Aarohi to extend their previous work to online learning setting.
Aarohi first trains an offline deep learning model with  log parsing, then utilizes grammar-based rules to provide online testing. Another approach from feature engineering tries to extract specific patterns about a certain time frame before a critical event.
This anomaly pattern can serve as a proactive alerts.
Klinkenberg \textit{et al.}~\cite{klinkenberg2017data} adopted descriptive statistics and supervised machine learning techniques to create such proactive alert from the system logs. They trained a binary classification model to detect the potential node failure based on a given time sequence of monitoring data collected from each node. 
% clustering-based
Berrocal \textit{et al.}~\cite{berrocal2014exploring} used environmental logs to extract numerical indicators and conducted a Void Search (VS) algorithm on these numerical values for the failure prediction task. 

\subsubsection{Heterogeneous Systems}  In heterogeneous systems, modeling the relationship among multiple components is the key, which is also the core part for the dominating relation mining algorithms.
% failure to outage
% Failures are regarded as abnormal signals detected by monitors and failure prediction is tackled from an anomaly detection point of view.
% critical failure
Different from homogeneous systems which focus on predicting failures based on raw signals sealed in the event logs or trace logs from single component, the prediction of critical failures (also called outage) in heterogeneous systems relies on the failure signals from log information collected from diversified system components.
In current real-time heterogeneous systems, such as the cloud system, outage prediction is an important and challenging task to perform. On one hand, outages are critical system failures that could lead to severe consequences.
On the other hand, outages occur without a significant alerting signals pattern, which makes it hard to predict. Moreover, the scope of impacting signals is a complex process to define.
% outages vs normal failure
Therefore, compared to homogeneous system settings, it is more valuable to detect node outages and distinguish regular internal failures from those caused by external factors, such as maintenance and human errors.

% methods
From the perspective of methodology, the advancement of failure prediction in heterogeneous systems relies on effective detection of the relationship between early alerting signals from system logs and node/component outage.
Chen \textit{et al.}~\cite{chen2019outage} proposed AirAlert framework based on Bayesian network to find the conditional dependence between the alerting signal extracted from system logs and the outage.
Then, given several alert signals, AirAlert employed gradient boosting tree method to conduct outage prediction.
Lin \textit{et al.}~\cite{lin2018predicting} designed MING framework to find the relationship between complex failure-indicating alerts and the outage from temporal and spatial features.
They carefully designed a ranking model that combines the intermediate results from LSTM model capturing temporal signals and a Random Forest model incorporating spatial data.
Zhou \textit{et al.}~\cite{zhou2019latent} proposed MEPFL to narrow down the scope of failure prediction into microservice level.
Based on a set of manual selected features defined on the system trace logs, MEPFL trains prediction models at both the trace level and the microservice level to predict three common types of microservice application faults: multi-instance faults, configuration faults, and asynchronous interaction faults.


\input{sections/failure_diagnosis}

\subsection{Others}
\label{sec:log_mining_others}

There are other valuable topics to broaden the log mining literature. In this section, we mainly introduce two reliability engineering tasks: specification mining and log-based software testing.

\subsubsection*{Specification Mining.}
Specification mining is the task of extracting specifications (e.g., program invariants) from program execution traces. Typical specifications impose constraints on the sequencing of program executions (ordering constraint) and program values (value constraint)~\cite{lo2007mining}. Such specifications play an important role in system comprehension, verification, and evolution. 
Ernst \textit{et al.}~\cite{ernst2007daikon,ernst2001dynamically} leveraged dynamic techniques to discover program invariants from execution traces. Specifically, they instrumented programs to write variables at critical program points (\textit{e.g.}, procedure entries and exits) and checked them against a series of potential invariant rules. They also released an open-source toolkit named Daikon~\cite{Daikon} for public reuse, which supports dynamic detection of likely invariants from program computes. Lo~\textit{et al.}~\cite{lo2007mining} mined modal scenario-based specifications in the framework of Damm and Harel’s Live Sequence Charts (LSC)~\cite{damm2001lscs} from execution traces, which describe the relations among caller/callee object identifier, and method signature. Lo \textit{et al.}~\cite{lo2008mining} further extended this model to explore the trigger-and-effect relationship of different charts in LSCs. Moreover, they found the combination of scenario-based and value-based specification mining is able to yield more rich specifications~\cite{lo2012scenario}.
Using the ITU-T standard Use Case Maps language, Hassine \textit{et al.}~\cite{hassine2018framework} visualized execution traces to recover availability scenarios. Such availability scenarios describe the degree to which a system or a component is operational and accessible.
In modern user-intensive applications, understanding user behaviors is crucial for their design. To this end, Ghezzi et al.~\cite{ghezzi2014mining} inferred a set of Markov models from user interaction logs to capture their behaviors probabilistically. Lemieux \textit{et al.}~\cite{lemieux2015general} introduced a tool named Texada to discover temporal behaviors of programs that hold true on log traces.

% \subsubsection*{Duplicate Issue Mining.}
% Developers may submit the same issue or bug report to the repository.
% These duplicate issue reports should be detected when new report arrives.
% Otherwise, issue maintainer will encounter heavy but unnecessary workload to process these reports.
% % via execution stack
% Wang \textit{et al.}~\cite{wang2008approach} uses classification techniques to detect duplicate issues with higher accuracy from informative execution traces as a reliable bug information source.
% Another important duplicate issue is duplicated logging statements.
% Developers cannot easily distinguish what is the occurred exception when analyzing the produced logs.
% Since developers rely on logs for debugging and program comprehension, such duplicate logging statements may negatively affect developers’ activities in maintenance and quality assurance.
% duplicate issue classification
% Ding \textit{et al.}~\cite{ding2014mining} transferred the duplicate-issue detection problem to similar context mining from the history records.
% They generated a signature for each issue from its corresponding transaction logs and then retrieved historical issues with similar signatures from a historical issue repository.~\slhe{to remove, and move one pub to another section.}

\subsubsection*{Log-based Software Testing.}
% software testing
Log-based software testing aims to stimulate the overall software workflow under testing by the generated log data.
Many existing work solves this problem by proposing a variety of state-machine-based formalism, similar to the techniques introduced in Section~\ref{sec:log_mining_workflow}. 
A pioneer work~\cite{andrews1998testing} discussed the availability of using formal log analyzer to enhance software reliability.
The majority of log-based testing approaches utilize cues from log files to improve testing coverage or completeness, 
Chen \textit{et al.}~\cite{chen2018automated} designed a framework called LogCoCo to estimate code coverage measures using the readily available execution logs.
Chen \textit{et al.}~\cite{chen2019experience} derived the state machine framework to conduct workload testing by extracting representative user behaviors from large-scale systems.
Cohen et al. \cite{cohen2015have} proposed a concept called log confidence to evaluate the completeness of any log-based dynamic specification mining task.

% \subsubsection*{Trace Checking}
% Tracing Back Log Data to its Log Statement: From Research to Practice~\cite{}



%% Diagnosis and debugging
% LOGAN: Problem Diagnosis in the Cloud Using Log-based Reference Models
% Gretel: Lightweight fault localization for openstack
% Log-based Abnormal Task Detection and Root Cause Analysis for Spark ICWS17

% Structured comparative analysis of systems logs to diagnose performance problems
% UiLog: Improving Log-Based Fault Diagnosis by Log Analysis
% An Empirical Study On Leveraging Logs For Debugging Production Failures
% (Association mining for logs, could be used for debugging) One graph is worth a thousand logs: Uncovering hidden structures in massive system event logs
% Log-based Abnormal Task Detection and Root Cause Analysis for Spark



%% Logging statements and practices
% Studying the characteristics of logging practices in mobile apps: a case study on F-Droid
% Studying and detecting log-related issues

%% Log parsing
% Efficient and robust syslog parsing for network devices in datacenter networks
% Aecid-pg: A tree-based log parser generator to enable log analysis
% X-trace: A Pervasive Network Tracing Framework
% Pip: Detecting The Unexpected In Distributed Systems
% (king of log parsing) LogMine: Fast Pattern Recognition for Log Analytics

%% Tools
% http://logsurfer.sourceforge.net
% https://www.elastic.co/cn/logstash
%  Amazon CloudWatch
% log4j

% Logentries https://docs.logentries.com/
% Loggly https://www.loggly.com/
% Splunk https://www.splunk.com/
% Sumo Logic https://www.sumologic.com/
% (OS) ELASTIC LOGS https://www.elastic.co/cn/log-monitoring
% (OS) Graylog https://www.graylog.org/
% (OS) OSSIM https://cybersecurity.att.com/products/ossim

%% Others
% User-assisted log analysis for quality control of distributed fintech applications


==> [CSUR 2020] Log Survey/sections/log_parsing.tex <==
\section{Log Parsing}
\label{sec:log_parsing}

\begin{figure}[t!]
\centering
\includegraphics[scale=0.5]{figs/parsingframework.pdf}
\caption{A log parsing example.}
\label{fig:parse}
\vspace{-5pt}
\end{figure}

After log collection, log messages will be input into different downstream log mining tasks (\textit{e.g.}, anomaly detection) for further analysis. However, most of the existing log mining tools~\cite{xu2009detecting, he2018identifying} require structured input data (\textit{e.g.}, a list of structured log events or a matrix). Thus, a crucial step of automated log analysis is to parse the semi-structured log messages into structured log events. 

% Section~\ref{sec:parse_def} introduces the input and output of log parsing and presents an example (Fig.~\ref{fig:parse}). Section~\ref{sec:parse_challenge} explains the challenges for log parsing. The two categories of existing log parsers are then introduced in Section~\ref{sec:parse_offline} (offline) and~\ref{sec:parse_online} (online).




Fig.~\ref{fig:parse} presents a log parsing example, where the input is a log message collected from Hadoop Distributed File System (HDFS)~\cite{xu2009detecting}. A log message is composed of message header and message content. The message header is determined by the logging framework and thus it is relatively easy to extract, such as verbosity levels (\textit{e.g.}, "INFO"). In contrast, it is difficult to extract key information from the message content because it is mainly written by developers in free-form natural language. Typically, the message content contains \textit{constants} and \textit{variables}. Constants are the fixed text written by the developers (\textit{e.g.}, "Received") and describe a system event, while variables are the values of the program variables which carry dynamic runtime information. The goal of log parsing is to distinguish between \textit{constants} and \textit{variables}. All the constants form the \textit{event template}. The output of a log parser is a structured log message, containing an event template and the key parameters.



\subsection{Challenges for Log Parsing}\label{sec:parse_challenge}
As a key component, log parsing has become an appealing selling-point~\cite{rapid_autoparsing,logz_autoparsing,loggly_autoparsing} of many industrial log management solutions~\cite{DBLP:conf/icse/ZhuHLHXZL19} (\textit{e.g.}, Splunk~\cite{splunk}). However, these industrial solutions only support common log types such as Apache logs~\cite{rapid_autoparsing}. When parsing general log messages, they rely on regexs and ad-hoc scripts provided by developers. These scripts separate log messages into different groups, where log messages in the same group have the same event template. In modern software engineering, even with these existing industrial solutions, log parsing is still a challenging task due to three main reasons: (1) the large volume of logs and thus the great effort on manual regex construction; (2) the complexity of software and thus the diversity of event templates; and (3) the frequency of software updates and thus the frequent update of logging statements.

% \subsubsection*{Volume of logs} As software is becoming much larger in scale (\textit{e.g.}, cloud systems), the volume of software logs has increased rapidly (\textit{e.g.}, 50 GB/h~\cite{mi2013toward}).

% \subsubsection*{Complexity of software} With the prevalence of Web service and source code sharing platform (\textit{e.g.}, Github), software could be written by hundreds of developers all over the world. Thus, developers who maintain the parsing regular expressions often have no idea of the original logging purpose, which further increase difficulty of log parsing.

% \subsubsection*{Frequency of software update} Because of the wide adoption of the agile software development concept, a new software version often comes in a short manner. Thus, the corresponding logging statements updates frequently as well (e.g, hundreds of new logging statement each month~\cite{weixutheis}). However, it is difficult for the developers to manually update the parsing regular expressions.



% \subsection{Problem Definition}\label{sec:parse_def}


\subsection{Log Parser Characteristics}
We explore 15 automated log parsing approaches. To provide a clear glimpse of these parsers, we focus on three main characteristics: mode, coverage, and preprocessing. We follow the definition introduced by Zhu \textit{et al.}~\cite{DBLP:conf/icse/ZhuHLHXZL19}. Note that different from their work, which was an evaluation study providing benchmarks and open-source implementation of existing log parsers, this survey focuses on the methodological comparison of these parsers. In addition, while parsing rules can be constructed by analyzing source code~\cite{xu2009detecting}, we focus on parsers that only utilize logs as input.

\subsubsection*{Mode} Mode is the most important log parsing characteristic to consider. Depending on the usage scenarios of parsing, log parsers can be categorized into two modes: offline and online. Offline log parsers require all the log messages beforehand and parse log messages in a batch manner. To cope with the frequent software update, developers need to periodically re-run the offline parser to obtain the newest event templates. In contrast, online parsers parse the log messages in a streaming manner, which work seamlessly with the downstream log mining tasks.

\subsubsection*{Coverage} We denote coverage as the capability of a log parser to match all input log messages with event templates. Note that this is orthogonal to whether the matched event templates are correct or not. In Table~\ref{tab:parsesum}, ``Partial" indicates the parser can only parse part of the log messages (\textit{i.e.}, some logs will be matched with no event templates). For example, SLCT~\cite{vaarandi2003data} matches a log message with an event template only if the log message contains a specific ``frequent pattern" and thus leaving the remaining log messages unparsed. Therefore, SLCT achieves “Partial” coverage. ``Partial" coverage might lead to the neglection of crucial system anomalies.

\subsubsection*{Preprocessing} Preprocessing removes some \textit{variables} or replaces them by \textit{constants} based on domain knowledge. For example, IP addresses (\textit{e.g.}, 10.251.42.84) are typical variables in cloud systems' log messages. This step requires some manual efforts (\textit{i.e.}, constructing regexs for these variables). 


% \begin{table}[h]
% \centering{}
% \caption{Summary of Log Parsing Approaches.}
% \includegraphics[scale=0.8]{figs/parserinfo.pdf}
% \label{tab:parsesum}
% \end{table}

\begin{table}[t]
\begin{center}
\caption{Summary of log parsing approaches.}
\label{tab:parsesum}
 \begin{tabular}{c|c|c|c|c}
 \toprule
\multicolumn{2}{c|}{\bf Methods} & Coverage & Preprocessing	& Technique	\\ \midrule
  \multirow{10}{*}{\rotatebox[origin=c]{90}{{\bf Offline}}} 
& SLCT~\cite{vaarandi2003data} & Partial	&  No	& Frequent pattern mining	 \\
& AEL~\cite{AEL_1}  & All	&  Yes	& Heuristics		\\
& LKE~\cite{qfu09} & All	&  Yes	& Clustering		 \\
& LFA~\cite{LFA_10}  & All	& No	& Frequent pattern mining	 \\
& LogSig~\cite{tang2011logsig} & All	&  No	& Clustering	 \\
& IPLoM~\cite{IPLoM09, IPLoM12} & All	&  No	& Iterative partitioning	 \\
& LogCluster~\cite{logcluster15} & Partial	&  No	& Frequent pattern mining	 \\
& LogMine~\cite{logmine16} & All	&  Yes	& Clustering	 \\
& POP~\cite{He2017TDSC} & All	&  Yes	& Iterative partitioning	 \\
& MoLFI~\cite{molfi18} & All	&  Yes	& Evolutionary algorithms	 \\

\midrule
  \multirow{5}{*}{\rotatebox[origin=c]{90}{{\bf Online}}} 
& SHISO~\cite{SHISO_13} & All	& No	& Clustering	 \\
& LenMa~\cite{lenma16} & All	  &  No	& Clustering		\\
& Spell~\cite{DuTKDE18}  & All	&  No	& Longest common subsequence	 \\
& Drain~\cite{He17ICWS, He2018Drain} & All	&  Yes	& Heuristics		\\
& Logram~\cite{Dai20Logram} & All	&  Yes	& Frequent pattern mining	 \\
\bottomrule

 \end{tabular} 
\end{center}
\vspace{-5pt}
\end{table} 

\subsection{Offline Log Parsing Approaches}\label{sec:parse_offline}

\subsubsection*{Frequent Pattern Mining} 
\textit{SLCT} (Simple Logfile Clustering Tool) \cite{vaarandi2003data} is the first research paper on automated log parsing. SLCT conducted two passes in total to obtain associated words. In the first pass, SLCT counted the occurrence of all the tokens and marked down the frequent words. These frequent words were utilized in the second pass to find out associated frequent words. Finally, for a log message, if it contained a pattern of associated frequent words, these words would be regarded as constants and employed to generate event templates. Otherwise, the log message would be placed into an outlier cluster without matched event templates.
\textit{LFA}~\cite{LFA_10} adopted a similar strategy as SLCT. Differently, LFA could cover all the log messages.


\subsubsection*{Clustering} \textit{LogCluster}~\cite{logcluster15} is similar to SLCT~\cite{vaarandi2003data}. Differently, LogCluster allowed variable length of parameters in between via a clustering algorithm. Thus, compared with SLCT, LogCluster is better at handling log messages of which the parameter length is flexible. For example, ``Download Facebook and install" and "Download Whats App and install" have the same event template ``Download <*> and install" while the length of the parameter (\textit{i.e.}, an app name) is flexible. \textit{LKE} (Log Key Extraction)~\cite{qfu09} was developed by Microsoft. LKE adopted a hierarchical clustering algorithms with a customized weighted edit distance metric. Additionally, the clusters were further partitioned by heuristic rules. \textit{LogSig} \cite{tang2011logsig} was a more recent clustering-based parser than LKE. Instead of directly clustering log messages, LogSig transformed each log message into a set of word pairs and clustered logs based on the corresponding pairs. \textit{LogMine}~\cite{logmine16} adopted an agglomerative clustering algorithm. It was implemented in map-reduce framework for better efficiency.

\subsubsection*{Heuristics} \textit{AEL}~\cite{AEL_1} employed a list of specialized heuristic rules. For example, for all the pairs like ``word=value," AEL regarded the ``value" as a variable and replaced it with a ``\$v" symbol. 

% Other heuristics include the number of words and parameters and typical natural language patterns (\textit{e.g.}, ``value" in ``is[are|was|were] value" is parameter).


\subsubsection*{Evolutionary Algorithms} \textit{MoLFI}~\cite{molfi18} formulate log parsing as a multi-objective optimization problem and propose an evolutionary algorithm-based approach. Specifically, MoLFI employs the Non-dominated Sorting Genetic Algorithm II~\cite{deb2002fast} to search for a Pareto optimal set of event templates. Compared with other log parsers, the strength of MoLFI is that it requires little parameter tuning effort because the four parameters required by MoLFI has effective default values. However, because of the adoption of evolutionary algorithm, the MoLFI is slower than most of the parsers.


\subsubsection*{Iterative Partitioning} \textit{IPLoM} \cite{IPLoM09, IPLoM12} contained three steps and partitioned log messages into groups in a hierarchical manner. (1) Partition by log message length. (2) Partition by \textit{token position}. The position containing the least number of unique words is ``token position". Partitioning was conducted according to the words in the token position. (3) Partition by mapping. Mapping relationships were searched between the set of unique tokens in two token positions, which were selected using a heuristic criterion. \textit{POP}~\cite{He2017TDSC} is a parallel log parser that utilizes distributed computing to accelerate the parsing of large-scale software logs. POP can parse 200 million HDFS log messages in 7 mins, while most of the parsers (\textit{e.g.}, LogSig) failed to terminate in reasonable time.

% Similar to IPLoM~\cite{IPLoM12}, the core concept of POP is iterative partitioning. Different from IPLoM that applies different heuristics, POP iteratively partitions the log messages based on \textit{token positions}. POP is implemented on top of Spark, a large-scale data processing platform. Due to its parallel algorithm design and implementation, 

\subsection{Online Log Parsing Approaches}\label{sec:parse_online}

\subsubsection*{Clustering} \textit{SHISO}~\cite{SHISO_13} is the first online log parsing approach. SHISO used a tree-form structure to guide the parsing process, where each node was correlated with a log group and an event template. The numbers of children nodes in all the layers were the same and were manually configured beforehand. During the parsing process, SHISO traversed the tree to find the most suitable log group by comparing the log message and the event templates in the corresponding log groups. SHISO is sensitive to path explosion and thus its efficiency is often unsatisfactory. \textit{LenMa}~\cite{lenma16} is similar to SHISO. LenMa encodes each log message into a \textit{length vector}, where each dimension records the number of characters of a token. For example, ``Receive a file." would be vectorized as [7, 1, 5]. During parsing, LenMa would compare the length vectors of the log messages.


\subsubsection*{Longest Common Subsequence} Similar to SHISO and LenMa, \textit{Spell}~\cite{DuTKDE18} maintained a list of log groups. To accelerate the parsing process, Spell utilized specialized data structures: prefix tree and inverted index. In addition, Spell provided a parallel implementation.


\subsubsection*{Heuristics} \textit{Drain}~\cite{He17ICWS} maintained log groups via the leaf nodes in the tree. The internal nodes of the tree embedded different heuristic rules. The extended version of Drain~\cite{He2018Drain} was based on a directed acyclic graph that allowed log group online merging. In addition, it provided the first automated parameter tuning mechanism for log parsing.

% In particular, each node in the first internal layer denotes a specific ``length" (number of tokens in a log message), where nodes in other internal layer denotes a specific constant. For example, assume that a node in the second internal layer denotes ``Received," then all log messages starting with token ``Received" will traverse through this node during online parsing.

\subsubsection*{Frequent Pattern Mining} \textit{Logram}~\cite{Dai20Logram} is the current state-of-the-art parser. Different from the existing approaches that count frequent tokens, Logram considered frequent n-gram. The core insight of Logram is: frequent n-gram are more likely to be constants. Note that Logram assumed developers had some log messages on hand to construct the dictionary.

% Logram conducts a pass through existing log messages to construct a dictionary of frequent 2-grams and 3-gram. After filtering some n-grams that may contain variables, the n-gram dictionary is used to generate event template for the log messages.

==> [CSUR 2020] Log Survey/sections/logging_practice.tex <==
\section{Logging}
\label{sec:log_practice}

% Describe the definition and application of logging.
Logging is the task of constructing logging statements with proper description and necessary program variables, and inserting the logging statements to the right positions in the source code. Logging has attracted attention from both academia~\cite{DBLP:conf/icse/PecchiaCCC15, ms-event-logging, DBLP:conf/dsn/SchroederG06, xu2009detecting} and industry~\cite{DBLP:journals/ese/ChenJ17, DBLP:conf/icse/FuZHLDLZX14, DBLP:conf/icse/PecchiaCCC15, DBLP:conf/icse/YuanPZ12, DBLP:journals/ese/ZengCSC19, DBLP:conf/icse/BarikDDF16} across a variety of application domains because logging is a fundamental step for all the subsequent log mining tasks. 

% However, logging practice is scarcely documented or regulated by strict standard, such as the logging mechanism and APIs~\cite{DBLP:conf/icse/BarikDDF16}. Essentially, logging is a subjective task that relies heavily on human expertise~\cite{DBLP:journals/cacm/OlinerGX12, DBLP:conf/icse/Shang12, DBLP:conf/icse/FuZHLDLZX14, DBLP:conf/icse/PecchiaCCC15, DBLP:conf/kbse/HeCHL18}. 

% Common aspects of logging statements, which will be minutely elaborated in Section~\ref{sec:logging-challenges}, include \emph{diagnosability}, \emph{maintenance}, \emph{performance}, \emph{security}, etc. 

% , such as execution tracing, debugging, state dump~\cite{DBLP:conf/icse/PecchiaCCC15}, event reporting~\cite{ms-event-logging}, error and failure characterization~\cite{DBLP:conf/dsn/SchroederG06}, anomaly detection~\cite{xu2009detecting}, and security analysis~\cite{DBLP:conf/nsdi/LamMV10, DBLP:conf/ndss/PaccagnellaDH0F20}

% In this section, we first define the basic mechanism of logging (Section~\ref{sec:logging-mechanism}), then review the challenges (Section~\ref{sec:logging-challenges}) and existing solutions (Section~\ref{sec:logging-solution}). 


\subsection{Logging Mechanism and Libraries} \label{sec:logging-mechanism}
% Describe how logs are generated in detail.

\subsubsection{Logging Mechanism}
Logging mechanism is the set of logging statements and their activation code implemented by developers or a given software platform~\cite{DBLP:conf/icse/PecchiaCCC15}. Fig.~\ref{fig:slf4j-example} shows two example logging statements and the collected logs during the execution of the program. The logging statement at line 3 is executed every time the \fixedwidth{setTemperature} method is called, with no specific activation code. The logging statement at line 5 is controlled by the activation code \fixedwidth{if (temperature.intValue() > 50)} at line 4. According to the data collected by~\cite{DBLP:conf/icse/PecchiaCCC15}, the most widely-adopted coding pattern that is used to activate the logging statements is \fixedwidth{if (condition) then log error()}.

% At line 3, the logging object is \fixedwidth{logger}, the verbosity level is \fixedwidth{debug}, the static texts are \fixedwidth{``Temperature set to'', ``Old temperature was''} and dynamic contents are \fixedwidth{t, oldT}.

\subsubsection{Logging Libraries}
To improve flexibility, industrial developers often utilizes logging libraries~\cite{DBLP:conf/icse/PecchiaCCC15, chen2020studying}, which are software components that facilitate logging and provide advanced features (\textit{e.g.}, thread-safety, log archive configuration, and API separation). Toward this end, a lot of open-source logging libraries have been developed (\textit{e.g.}, Log4j~\cite{Log4j}, SLF4J~\cite{SLF4J}, AspectJ~\cite{AspectJ}, spdlog~\cite{spdlog}). 

% Chen \textit{et al.}~\cite{chen2020studying} conducted a large-scale empirical study on the practices of Java logging libraries adoption in GitHub.

% Log4j\footnote{\url{http://logging.apache.org/log4j/}} and SLF4J\footnote{\url{http://www.slf4j.org/}} are popular logging libraries for Java. SLF4J serves as a simple and flexible abstraction for various logging frameworks (\textit{e.g.} Log4j, a fully-fledged logging library from Apache Software Foundation). AspectJ\footnote{\url{https://www.eclipse.org/aspectj/}} is an aspect-oriented extension of Java, which we will further introduce in Section~\ref{sec:practice-maintenance}. spdlog\footnote{\url{https://github.com/gabime/spdlog}} is a very fast cross-platform logging library written in C++11. It has an asynchronous mode, multi-threaded logging, rich formatting, and a lot more features.


\subsection{Challenges for Logging} \label{sec:logging-challenges}

% TODO: Describe more about what industry need (the aim of logging)

Logging in a software system is usually decided by an empirical process in the development phase~\cite{DBLP:conf/icse/PecchiaCCC15}. In general, logging practice, \textit{i.e.}, how developers conduct the task of logging, is scarcely documented or regulated by strict standard, such as the logging mechanism and APIs~\cite{DBLP:conf/icse/BarikDDF16}. Thus, logging relies heavily on human expertise~\cite{DBLP:journals/cacm/OlinerGX12, DBLP:conf/icse/Shang12, DBLP:conf/icse/FuZHLDLZX14, DBLP:conf/icse/PecchiaCCC15, DBLP:conf/kbse/HeCHL18}. In the following, we summarize three main challenges for automated logging, which also align with the taxonomy mentioned by Chen and Jiang~\cite{DBLP:conf/icse/ChenJ17}: \emph{where-to-log}, \emph{what-to-log}, and \emph{how-to-log}. Under this categorization, every problem exhibits aspects that represent the primary concerns of the actual practice of logging. Accordingly, we summarize three major aspects, \textit{i.e.}, \emph{diagnosability}, \emph{maintenance}, and \emph{performance}.

% , and \emph{security}.

% Therefore, understanding the challenges underlying logging is crucial for establishing effective logging statements and mechanism. 


\subsubsection{where-to-log}

Where-to-log is about determining the appropriate location of logging statements. Although logging statements provide rich information and can be inserted almost everywhere, excessive logging results in performance degradation~\cite{DBLP:conf/icse/ChenJ17} and incurs additional maintenance overhead. In addition, it is challenging to diagnose problems by analyzing a large volume of logs as most logs are unrelated to the problematic scenarios~\cite{DBLP:conf/icsm/JiangHHF08}. On the other hand, insufficient logging will also impede the logs' diagnosability. For example, an incomplete sequence of logs may hinder the reproduction of precise execution paths~\cite{DBLP:conf/sosp/ZhaoRLSYZ17}.
% The absence of logging statements in the exception block leads to incomplete fault information, making fault diagnosis more difficult~\cite{DBLP:conf/osdi/YuanPHLLTZS12}.
Therefore, developers need to be circumspect in their choices of where-to-log.


\subsubsection{what-to-log}

What-to-log is about providing sufficient and concise information within the three major components of a logging statement, \textit{i.e.}, verbosity level, static text, and dynamic content. Mis-configured verbosity level has similar consequences with inappropriate logging points. As developers typically filter logs according to the verbosity levels, under-valued verbosity levels may result in missing or ignored log messages while over-valued verbosity levels lead to overwhelming log messages~\cite{DBLP:conf/icsm/JiangHHF08}. When composing a snippet of logging code, the static text should be concise and the dynamic content should be coherent and up-to-date. Poorly written static text and inconsistent dynamic content could affect the subsequent diagnosis and maintenance activities~\cite{DBLP:conf/msr/KabinnaBSH16, liu2019variables,zhang2019robust,meng2019loganomaly}.


\subsubsection{how-to-log}

% icse17chen
How-to-log is the "design pattern" and maintenance of logging statements systematically. Most software testing techniques focus on verifying the quality of feature code, but a few papers~\cite{DBLP:conf/icse/YuanPZ12, DBLP:journals/ese/ChenJ17, DBLP:conf/icse/ChenJ17,DBLP:journals/ese/HassaniSST18, DBLP:journals/ese/ShangNH15} pay attention to the quality and anti-patterns in the logging code. 
% Although the Aspect-Oriented Programming (AOP) paradigm~\cite{kiczales1997aspect} provides a systematic approach to modularize the logging statements, 
Most industrial and open source systems choose to scatter logging statements across the entire code base, intermixing with feature code~\cite{DBLP:conf/icse/ChenJ17}, which also hardens the maintenance of logging code.
% Bad logging code hinder program understanding or even cause runtime issues like crashes. % https://issues.apache.org/jira/browse/HBASE-750/


\subsection{Logging Approaches} \label{sec:logging-solution}

% This style looks better
\begin{table}[t]
  \centering
  \caption{Summary of logging approaches.}
  \label{tab:practice}
  \begin{tabular}{@{}l|l|p{8cm}@{}}
  \toprule
  \textbf{Problems}             & \textbf{Aspects} & \textbf{Objectives}  \\
  \midrule
  \multirow{4}{*}{\textbf{where-to-log}} & Diagnosability   & Suggest appropriate placement of logging statements into source code~\cite{DBLP:conf/dsn/CinqueCNP10,DBLP:conf/osdi/YuanPHLLTZS12,DBLP:journals/tse/CinqueCP13,DBLP:conf/icse/ZhuHFZLZ15, li2020wherelog,DBLP:conf/hotos/ZhaoRLSYZ17, DBLP:conf/sosp/ZhaoRLSYZ17, DBLP:journals/ese/YaoPSSTS20} ; Study logging practices in industry~\cite{DBLP:conf/icse/FuZHLDLZX14, DBLP:journals/ese/LiCSH18}.  \\
                                & Performance      & Minimize or reduce performance overhead~\cite{DBLP:conf/osdi/YuanPHLLTZS12, DBLP:conf/usenix/DingZLZLFZX15}.    \\
  \midrule
  \multirow{9}{*}{\textbf{what-to-log}}  & Diagnosability   & Enhance existing logging code to aid debugging~\cite{DBLP:conf/asplos/YuanZPZS11}; Suggest proper variables and text description in log~\cite{DBLP:conf/kbse/HeCHL18,liu2019variables, li2017log}.   \\
                                & Maintenance      & Determine whether a logging statement is likely to change in the future~\cite{DBLP:journals/ese/KabinnaBSSH18}; Characterize and detect duplicate logging code~\cite{DBLP:conf/icse/LiC0S19}.  \\
                                & Performance      & Study the performance overhead and energy impact of logging in mobile app~\cite{DBLP:journals/ese/ChowdhuryNHJ18, DBLP:journals/ese/ZengCSC19}; Automatically change the log level of a system in case of anomaly~\cite{DBLP:conf/iwpc/MizouchiSII19}.  \\
  \midrule
  \multirow{14}{*}{\textbf{how-to-log}}   & Diagnosability   & Characterize the anti-patterns in the logging code~\cite{DBLP:conf/icsm/ShangNHJ14}; Optimize the implementation of logging mechanism to facilitate failure diagnosis~\cite{DBLP:conf/usenix/LuoNSMC18}. \\
                                & Maintenance      & Characterize and detect the anti-patterns in the logging code~\cite{DBLP:conf/icse/YuanPZ12, DBLP:journals/ese/ChenJ17, DBLP:conf/icse/ChenJ17,DBLP:journals/ese/HassaniSST18, li2017towards, DBLP:journals/ese/LiNJLWL20}; Characterize and prioritize the maintenance of logging statements~\cite{DBLP:conf/msr/KabinnaBSH16}; Study the relationship between logging characteristics and the code quality~\cite{DBLP:journals/ese/ShangNH15, chen2019extracting}; Propose new abstraction or programming paradigm of logging~\cite{kiczales1997aspect,DBLP:conf/osdi/LockermanFKSAA018}.  \\
                                & Performance      & Optimize the compilation and execution of logging code~\cite{DBLP:conf/usenix/YangPO18}. \\
                                % & Security         & Mitigate the flood attack of access logs~\cite{DBLP:conf/nsdi/LamMV10}; Detect and prevent tampering in system logs for system auditing~\cite{DBLP:conf/ndss/PaccagnellaDH0F20}.  \\
  \bottomrule
  \end{tabular}
\end{table}

Numerous solutions have been proposed to address the challenges mentioned in Section~\ref{sec:logging-challenges}. Table~\ref{tab:practice} summarizes existing studies along with corresponding problems and aspects. Each row represents a challenge. The approaches fall into three categories: \textit{static code analysis}, \textit{machine learning}, and \textit{empirical study}. A bunch of early work utilized static code analysis to analyze logging in a program without executing the source code. Machine learning-based approaches focus on learning from data. By concentrating on the inherent statistical properties of existing logging statements, learning-based approaches automatically give suggestions on improving the logging statements. In the remainder of this section, we discuss solutions by their aspects.


\subsubsection{Diagnosability}

Logs are valuable for investigating and diagnosing failures. However, a logging statement is only as helpful as the information it provides. The research on this aspect aims at (1) understanding the helpfulness of logs for failure diagnosis and (2) making logs informative for diagnosis.

\par{\textit{(1) Understanding the helpfulness of logs for failure diagnosis.}}
This is of great importance because logs are widely adopted for failure diagnosis. According to a survey~\cite{DBLP:conf/icse/FuZHLDLZX14} involving 54 experienced developers in Microsoft, almost all the participants agreed that ``logging statements are important in system development and maintenance'' and ``logs are a primary source for problem diagnosis''. Fu \textit{et al.}~\cite{DBLP:conf/icse/FuZHLDLZX14} also studied the types of logging statements in industrial software systems by source code analysis, and summarized five types of logging snippets, \textit{i.e.}, assertion-check logging, return-value-check logging, exception logging, logic-branch logging, and observing-point logging. Besides, Fu \textit{et al.}~\cite{DBLP:conf/icse/FuZHLDLZX14} further demonstrated the potential feasibility of predicting where to log.
%
Shang \textit{et al.}~\cite{DBLP:conf/icsm/ShangNHJ14} conducted the first empirical study to provide a taxonomy for user inquiries of logs. 
% By manually going through emails in the mailing list and StackOverflow questions for Hadoop, Cassandra and Zookeeper, 
They identified five types of information that were often sought from log lines by practitioners, \textit{i.e.}, meaning, cause, context, impact, and solution. Shang \textit{et al.}~\cite{DBLP:conf/icsm/ShangNHJ14} were also the first to associate the development knowledge at present in various development repositories (\textit{e.g.}, code commits and issues reports) with the log lines and to assist practitioners in resolving real-life log inquiries. In addition, Li \textit{et al.}~\cite{DBLP:journals/ese/LiCSH18} highlighted the feasibility of guiding developers' logging practice with topic models by investigating six open source systems.

\par{\textit{(2) Making logs informative for failure diagnosis.}}
As printed logs are often the only run-time information source for debugging and analysis, the quality of log data is critically important. \emph{LogEnhancer}~\cite{DBLP:conf/asplos/YuanZPZS11} made the first attempt to systematically and automatically augment existing logging statements in order to reduce the number of possible code paths and execution states for developers to pinpoint the root cause of a failure. Zhao \textit{et al.}~\cite{DBLP:conf/hotos/ZhaoRLSYZ17, DBLP:conf/sosp/ZhaoRLSYZ17} followed the idea of \emph{LogEnhancer} and proposed an algorithm capable of completely disambiguating the call path of HDFS requests. Yuan \textit{et al.}~\cite{DBLP:conf/osdi/YuanPHLLTZS12} found that the majority of unreported failures were manifested via a generic set of error patterns (\textit{e.g.}, system call return errors) and proposed the tool \emph{Errlog} to proactively add pattern-specific logging statements by static code analysis.

% rule based
As modern software becomes more complex, where-to-log has become an important but difficult decision, largely limited to the developer's domain knowledge. Around 60\% of failures due to software faults do not leave any trace in logs, and 70\% of the logging pattern aims to detect errors via a checking code placed at the end of a block of instructions~\cite{DBLP:conf/dsn/CinqueCNP10,DBLP:journals/tse/CinqueCP13}. Cinque \textit{et al.}~\cite{DBLP:journals/tse/CinqueCP13} concluded that the traditional logging mechanism has limited capacity due to the lack of a systematic error model. They further formalized the placement of the logging instruction and proposed to use system design artifacts to manually define \emph{rule-based logging} which utilizes error models about what cause errors to fail.
% learning
Zhu \textit{et al.}~\cite{DBLP:conf/icse/ZhuHFZLZ15} made an important first step towards the goal of ``learning to log''. They proposed a logging recommendation tool, \emph{LogAdvisor}, that learns the common logging rules on where-to-log from existing code via training a classifier and further leverages it for informative and viable recommendations to developers. Yao \textit{et al.}~\cite{DBLP:journals/ese/YaoPSSTS20} leveraged a statistical performance model to suggest the need for updating logging locations for performance monitoring. Li \textit{et al.}~\cite{li2020wherelog} proposed a deep learning framework to suggest where-to-log at the block level. Li \textit{et al.} also concluded that there might be similar rules regarding the implementation of logging mechanism across different systems and development teams, which agreed with the industrial survey by Pecchia \textit{et al.}~\cite{DBLP:conf/icse/PecchiaCCC15}.

The lack of strict logging guidance and domain-specific knowledge makes it difficult for developers to decide what-to-log. To address this need, Li \textit{et al.}~\cite{li2017log} employed ordinal regression model to suggest proper verbosity level based in software metrics. He \textit{et al.}~\cite{DBLP:conf/kbse/HeCHL18} conducted the first empirical study on the usage of natural language in logging statements. They showed the global (\textit{i.e.}, in a project) and local (\textit{i.e.}, in a file) repeatability of text descriptions. Furthermore, they demonstrated the potential of automated description text generation for logging statements. Liu \textit{et al.}~\cite{liu2019variables} proposed a deep learning-based approach to recommend variables in logging statements by learning embeddings of program tokens.
% from existing logging statements. 
In order to troubleshoot transiently-recurring problems in cloud-based production systems, Luo \textit{et al.}~\cite{DBLP:conf/usenix/LuoNSMC18} put forward a new logging mechanism that assigns a blame rank to methods based on their likelihood of being relevant to the root cause of the problem. With the blame rank, logs generated by a method over a period of time are proportional to how often it is blamed for various misbehavior, thus facilitating diagnosis.

% Jitsumoto \textit{et al.}~\cite{DBLP:conf/dsn/JitsumotoTIS14} (this is for fault tolerance in clusers)


\subsubsection{Maintenance} \label{sec:practice-maintenance}

The maintenance of logging code has also attracted researchers' interest. The research on this aspect aims at (1) characterizing the maintenance and detecting anti-patterns of logging statements and (2) proposing new abstractions of logging.

\par{\textit{(1) Characterizing the maintenance and detecting anti-patterns of logging statements.}}
Anti-patterns in logging statements are bad coding patterns that undermine the quality and effectiveness of logging statements and increases the maintenance effort of projects. Many papers~\cite{DBLP:journals/ese/ShangNH15, DBLP:journals/ese/ChenJ17, DBLP:journals/ese/HassaniSST18, chen2019extracting} performed empirical studies to reveal the link between logs and defects. These papers observed a positive correlation between logging characteristics and post-release defects. Therefore, practitioners should allocate more effort to source code files with more logging statements.

Yuan \textit{et al.}~\cite{DBLP:conf/icse/YuanPZ12} made the first attempt to conduct a quantitative characteristic study of how developers log within four pieces of large open-source software. They described common anti-patterns and provided insights into where developers spend most of their efforts in modifying the log messages and how to improve logging practice. They further implemented a prototype checker to verify the feasibility of detecting unknown problematic statements using historical commit data. Chen and Jiang~\cite{DBLP:conf/icse/ChenJ17} and Hassani \textit{et al.}~\cite{DBLP:journals/ese/HassaniSST18} both studied the problem of how-to-log by characterizing and detecting the anti-patterns in the logging code. The analysis~\cite{DBLP:conf/icse/ChenJ17} of well-maintained open-source systems revealed six anti-patterns that are endorsed by developers. Chen and Jiang~\cite{DBLP:conf/icse/ChenJ17} then encoded these anti-patterns into a static code analysis tool to automatically detect anti-patterns in the source code. Li \textit{et al.}~\cite{DBLP:conf/icse/LiC0S19} developed an automated static analysis tool, \emph{DLFinder}, to detect duplicate logging statements that have the same static text description.
% , which is also a kind of anti-pattern.

Just like feature code, logging code updates with time~\cite{DBLP:journals/ese/KabinnaBSSH18}. Moreover, logging statements are often changed without consideration for other stakeholders, resulting in sudden failures of log analysis tools and increased maintenance costs for such tools. Pecchia \textit{et al.}~\cite{DBLP:conf/icse/PecchiaCCC15} reviewed the industrial practice in the reengineering of logging code.
% by source code analysis, manual inspection of log entries, and direct feedback from developers. 
Kabinna \textit{et al.}~\cite{DBLP:conf/msr/KabinnaBSH16} empirically studied the migration of logging libraries and the main reasons for the migration. Li \textit{et al.}~\cite{li2017towards} derived and used a set of measures to predict whether a code commit requires log changes. Kabinna \textit{et al.}~\cite{DBLP:journals/ese/KabinnaBSSH18} later examined the important metrics for determining the stability of logging statements and further leveraged learning-based models (random forest classifier and Cox proportional hazards) to determine whether a logging statement is likely to remain unchanged in the future. Their findings were helpful to build robust log analysis tools by ensuring that these tools relied on logs generated by more stable logging statements. Li \textit{et al.}~\cite{DBLP:journals/ese/LiNJLWL20} designed a tool to learn log revision rules from logging context and modifications and recommend candidate log revisions.

\par{\textit{(2) Proposing new abstractions of logging.}}
Maintaining logging code along with feature code has proven to be error-prone~\cite{DBLP:journals/ese/ShangNH15, DBLP:journals/ese/ChenJ17, DBLP:journals/ese/HassaniSST18}. Hence, additional logging approaches~\cite{kiczales1997aspect, DBLP:conf/osdi/LockermanFKSAA018} have been proposed to resolve this issue. Kiczales \textit{et al.}~\cite{kiczales1997aspect} proposed a new programming paradigm that improves the modularity of the logging code. To tackle the ordering problem of logs in distributed systems, Lockerman \textit{et al.}~\cite{DBLP:conf/osdi/LockermanFKSAA018} introduced \emph{FuzzyLog} that featured strong consistency, durability, and failure atomicity.


\subsubsection{Performance}

The intermixing nature of the logging code and feature code usually incurs performance overhead, storage cost, and development and maintenance efforts~\cite{DBLP:conf/usenix/DingZLZLFZX15, DBLP:conf/asplos/YuanZPZS11, DBLP:conf/iwpc/MizouchiSII19, DBLP:journals/ese/ChowdhuryNHJ18, DBLP:journals/ese/ZengCSC19}. Tools like \emph{LogEnhancer}~\cite{DBLP:conf/asplos/YuanZPZS11}, \emph{Errlog}~\cite{DBLP:conf/osdi/YuanPHLLTZS12}, \emph{Log2}~\cite{DBLP:conf/usenix/DingZLZLFZX15}, and \emph{INFO-logging}~\cite{DBLP:conf/hotos/ZhaoRLSYZ17} all took performance into consideration while dealing with diagnosability and maintenance issues. Mizouchi \textit{et al.}~\cite{DBLP:conf/iwpc/MizouchiSII19} proposed a dynamical adjusting verbosity level to record irregular events while reducing performance overhead. Yang \textit{et al.}~\cite{DBLP:conf/usenix/YangPO18} proposed \emph{NanoLog}, a nanosecond scale logging system that achieved relatively low latency and high throughput by moving the workload of logging from the runtime hot path to the post-compilation and execution phases of the application. Chowdhury \textit{et al.}~\cite{DBLP:journals/ese/ChowdhuryNHJ18} were the first to explore the energy impact of logging in mobile apps. Zeng \textit{et al.}~\cite{DBLP:journals/ese/ZengCSC19} conducted a case study that characterized the performance impact of logging on Android apps.

% Another common and significant research topic about logs is security.  This topic focuses on making logging statements invulnerable and mitigating attacks by the logging mechanism. For instance, Lam \textit{et al.}~\cite{DBLP:conf/nsdi/LamMV10} proposed \emph{Carousel} to mitigate the flood attack of hundreds of millions of duplicate log records. Recently, Paccagnella \textit{et al.}~\cite{DBLP:conf/ndss/PaccagnellaDH0F20} introduced a practical framework, \emph{CUSTOS}, for the detection of tampering in system logs. System security is a central concern but it is beyond the scope of this paper so we will not go into this topic too much.

  


==> [CSUR 2020] Log Survey/sections/open_tools.tex <==
\section{Open-source Toolkits and Datasets}
\label{sec:log_tools}

\begin{table}[t]
\begin{center}
\caption{A list of open-source log analysis tools and log datasets.}
\label{table:log_tools}
 \begin{tabular}{c|c|c|c}
 \toprule
 \multicolumn{2}{c|}{\bf Category}  & Description & Link \\
  \midrule
\multirow{8}{*}{{\rotatebox[origin=c]{90}{\bf Tools}}} 
  & GrayLog & A centralized log collection and real-time analysis tool. & \cite{GrayLog} \\
  & GoAccess &  A real-time terminal-based log analyzer for web logs. &  \cite{GoAccess} \\
  & Fluentd & A data collector that unifies multiple logging infrastructures.  &\cite{Fluentd}  \\
 & Logstash & A server-side processor that ingests and transforms log data.  &\cite{Logstash}  \\
 & Logalyze & A centralized log management and network monitoring software. & \cite{Logalyze} \\
 & Prometheus & A monitoring solution for metrics collection and alerting. &\cite{Prometheus} \\
 & Syslog-ng & A scalable log collector and processor across infrastructures.&\cite{Syslog-ng}  \\
 & LogPAI & A comprehensive automated log analysis toolkit &\cite{LogPAI}  \\
 \midrule
\multirow{5}{*}{{\rotatebox[origin=c]{90}{\bf Datasets}}}
  & Loghub & A large collection of log datasets from various systems. &\cite{Loghub}  \\
  & Failure dataset& Error logs produced by OpenStack cloud system. & \cite{failure_data} \\
  & CFDR & Computer failure data repository of different systems. &\cite{CFDR}  \\
  & SecRepo & A list of security log data such as malware and system logs. &\cite{SecRepo}\\
  & EDGAR & Apache log files that record and store user access statistic. &\cite{EDGAR}  \\
  \bottomrule
 \end{tabular} 
\end{center}
\vspace{-4pt}
\end{table} 


% & GrayLog & A centralized log collection and real-time analysis tool. & \href{https://www.graylog.org}{link} \\
%   & GoAccess &  A real-time terminal-based log analyzer for web logs. &  \href{https://goaccess.io}{link} \\
%   & Fluentd & A data collector that unifies multiple logging infrastructures.  & \href{https://www.fluentd.org}{link} \\
%  & Logstash & A server-side processor that ingests and transforms log data.  & \href{https://www.elastic.co/logstash}{link} \\
%  & Logalyze & A centralized log management and network monitoring software. & \href{http://www.logalyze.com}{link} \\
%  & Prometheus & A monitoring solution for metrics collection and alerting. &\href{https://github.com/prometheus}{link} \\
%  & Syslog-ng & A scalable log collector and processor across infrastructures.& \href{https://www.syslog-ng.com}{link} \\
%  & LogPAI & A comprehensive automated log analysis toolkit & \href{https://www.logpai.com}{link} \\
%  \midrule
% \multirow{5}{*}{{\rotatebox[origin=c]{90}{\bf Datasets}}}
%   & Loghub & A large collection of log datasets from various systems. & \href{https://github.com/logpai/loghub/}{link} \\
%   & Failure dataset& Error logs produced by OpenStack cloud system. & \href{https://figshare.com/articles/Failure_dataset/7732268/2}{link} \\
%   & CFDR & Computer failure data repository of different systems. & \href{https://www.usenix.org/cfdr}{link} \\
%   & SecRepo & A list of security log data such as malware and system logs. & \href{http://www.secrepo.com}{link}\\
%   & EDGAR & Apache log files that record and store user access statistic. & \href{https://www.sec.gov/dera/data/edgar-log-file-data-set.html}{link} \\



In recent years, there are many research studies focusing on automated log analysis. Meanwhile, a number of log management tools have been developed to facilitate the real-world deployment in industry. In this section, we review existing open-source tools and datasets for automated log analysis. To select the desired tools, we define the following criteria: First, we did not consider commercial log analysis tools, such as Splunk~\cite{splunk} and Loggly~\cite{loggly}; Second, the selected tools should cover multiple log analysis phases presented in the paper. After carefully searching, we curated a list of open-source log analysis toolkits, as shown in Table~\ref{table:log_tools}. These log analysis tools are GrayLog, GoAccess, Fluentd, Logstash, Logalyze, Prometheus, Syslog-ng, and LogPAI. In common, these tools support crucial features such as log collection, searching, routing, parsing, visualization, alerting and automated analysis. Among these tools, LogPAI is an open-source project built upon pure research outputs while other tools are packed as open-source enterprise products. Additionally, most of existing tools focus on phases before the log mining (\textit{e.g.}, log parsing), and the resulting outcomes (\textit{e.g.}, visualization) are presented to developers for manual analysis. Particularly, LogPAI provides a set of automated log analysis tools such as log parsing and anomaly detection.
% 




% \begin{table}[t]
% \begin{center}
% \caption{A list of public log datasets.}
% \label{table:log_data}
%  \begin{tabular}{c|c|c}
%  Datasets & Description & Link \\
%   \hline  \hline
%   Loghub & A comprehensive collection of log datasets from various systems. & \href{https://github.com/logpai/loghub/}{link} \\
%   Failure dataset& Error logs produced by the OpenStack cloud management system. & \href{https://figshare.com/articles/Failure_dataset/7732268/2}{link} \\
%   CFDR & Computer failure data repository of different systems. & \href{https://www.usenix.org/cfdr}{link} \\
%   SecRepo & A list of security log data such as malware and system logs. & \href{http://www.secrepo.com}{link}\\
%   EDGAR & Apache log files that record and store user access statistic. & \href{https://www.sec.gov/dera/data/edgar-log-file-data-set.html}{link} \\
%   \hline
%  \end{tabular} 
% \end{center}
% \end{table} 


Besides the open-source toolkits, a number of log datasets collected from various software systems are available for research studies in academia. Table~\ref{table:log_tools} shows the list of public log datasets and their descriptions. The  Loghub~\cite{he2020loghub} maintains a large log collection that is freely accessible for research purposes. Some log datasets are production data released from previous studies, while others are collected in the lab environment. Another research study~\cite{cotroneo2019bad} presented error logs produced by injecting failures in the OpenStack cloud management system. The computer failure data repository (CFDR) focuses mainly on component failure logs in a variety of large production systems. Besides these log datasets, there are also logs collected for other purposes, such as security and web search. SecRepo is a curated list of security data such as malware and system logs.  The EDGAR dataset contains Apache logs that record user access statistic through internet search. 

==> [CSUR 2020] Log Survey/sections/survey_method.tex <==
\section{Survey Methodology}

\begin{figure}[t!]
\centerline{\includegraphics[width=0.90\columnwidth]{figs/dist_year.pdf}}
\caption{Paper distribution on each research topic and the associated evolution trend from 1997 to 2020.}
\label{fig:dist_year}
\vspace{-2pt}
\end{figure}


To systematically collect the publications for conducting this survey, we maintained a repository for the automated log analysis literature. We first searched relevant papers in online digital libraries and extended the repository by manually inspecting all references of these papers. The repository is now available online.\footnote{\url{https://github.com/logpai/awesome-log-analysis}}


To begin with, we searched several popular online digital libraries (\textit{e.g.}, IEEE Xplore, ACM Digital Library, Springer Online, Elsevier Online, Wiley Online, and ScienceDirect) with the following keywords: "log", "logging", "log parsing", "log compression", "log + anomaly detection", "log + failure prediction", "log + failure diagnosis". The "log" term is broadly quoted in various domains, such as the query log in database, web search log in recommendation, and the logarithm function in mathematics. Hence, to precisely collect the set of papers of our interest, we mainly focused on regular papers published in top venues (\textit{i.e.}, conferences and journals) of relevant domains, including ICSE, FSE, ASE, TSE, TOSEM, EMSE, SOSP, OSDI, ATC, NSDI, TDSC, DSN, ASPLOS, and TPDS. 
Then, we manually inspected each reference of these papers to collect additional publications that are related to the survey topics. In this paper, we focused on publications studying the reliability issues with software system logs, while publications of other topics are beyond the scope of this survey, such as logs for security and privacy~\cite{king2017log}, software change logs~\cite{chen2004open}, kernel logs~\cite{paccagnella2020custos}, and process mining logs~\cite{van2012process}.

In total, we collected 158 publications in automated log analysis area spanning from year 1997 to 2020. Fig.~\ref{fig:dist_year} (on the right part) shows the histogram of annual publications during the period. We can find that automated log analysis has been continuously and actively investigated in the past two decades. In particular, we can observe steady growth in the number of publications since 2006, indicating that the log analysis field has attracted an increasing amount of interest since then. 
% \textcolor{red}{It is also partially because of the increasing number of research studies in software engineering area~\cite{software_trend}.}
% One possible reason is that the prosperity of cloud computing leads to the high demand of automated log analysis.

Furthermore, we classify these publications into five categories by research focus: logging, log compression, log parsing, log mining, and empirical study. The distribution is presented on the left part of  Fig.~\ref{fig:dist_year}. Note that some papers may address more than one research focuses, in which case we categorized the paper based on its major contribution. As expected, Fig.~\ref{fig:dist_year} shows that a large portion (around a half) of research efforts were devoted to log mining. The reasons are two-fold: First, log mining is a comprehensive task that consists of many sub-tasks (\textit{e.g.}, anomaly detection, failure diagnosis). Each sub-task has a huge space for research exploration and thereby attracts many research studies on it; Second, research areas other than log mining are relatively mature. Besides, logging is also extensively studied in the past decades since it is more closely related to industrial practices. In addition, many log research tasks are empirical studies, and we discussed them in different sections respectively.


Furthermore, we were aware of several existing surveys on logs analysis. Oliner \textit{et al.}~\cite{DBLP:journals/cacm/OlinerGX12} briefly reviewed sixteen log analysis papers and pointed out some challenges in 2012. Since then, the log analysis area has been actively studied, which impels a more comprehensive and systematic log survey paper. Other existing surveys mainly studied logs and their use in the security area. Khan \textit{et al.}~\cite{khan2016cloud} focused on logs in the  cloud computing environment and the logs were leveraged for identifying and preventing suspicious attacks. Zeng \textit{et al.}~\cite{zeng2016computer} studied the logging mechanisms and security issues in three computer operating systems. A recent publication~\cite{landauer2020system} reviewed clustering based approaches in cyber security applications. Different from these studies, our survey mainly targets the automated log analysis for tackling the general reliability issues. 







% \begin{figure}[th]
% \centerline{\includegraphics[width=0.6\columnwidth]{figs/distribution.pdf}}
% \caption{Paper distribution on each research topic in the literature on automated log analysis.}
% \label{fig:distribution}
% \end{figure}
